A Survey of Graph Pre-processing Methods: From Algorithmic to Hardware Perspectives

Graph-related applications have experienced significant growth in academia and industry, driven by the powerful representation capabilities of graph. However, efficiently executing these applications faces various challenges, such as load imbalance, random memory access, etc. To address these challenges, researchers have proposed various acceleration systems, including software frameworks and hardware accelerators, all of which incorporate graph pre-processing (GPP). GPP serves as a preparatory step before the formal execution of applications, involving techniques such as sampling, reorder, etc. However, GPP execution often remains overlooked, as the primary focus is directed towards enhancing graph applications themselves. This oversight is concerning, especially considering the explosive growth of real-world graph data, where GPP becomes essential and even dominates system running overhead. Furthermore, GPP methods exhibit significant variations across devices and applications due to high customization. Unfortunately, no comprehensive work systematically summarizes GPP. To address this gap and foster a better understanding of GPP, we present a comprehensive survey dedicated to this area. We propose a double-level taxonomy of GPP, considering both algorithmic and hardware perspectives. Through listing relavent works, we illustrate our taxonomy and conduct a thorough analysis and summary of diverse GPP techniques. Lastly, we discuss challenges in GPP and potential future directions.

==> old/background_old.tex <==
%在本节中，我们首先介绍图处理的背景，然后概述现有的图预处理方法。 最后，我们提出了图预处理方法的分类。 为了更好地说明我们的分类法，我们分析了硬件级别的图处理挑战并从中总结了优化目标。 我们根据优化目标将预处理方法分为三类：efficient computing，efficient storage，efficient communication的方法。
In this section, we first introduce the background of graph processing, and then give an outline of existing graph preprocessing methods. Last, we propose our taxonomy of graph preprocessing methods. To better illustrate our taxonomy, we analyze the challenges of graph processing in hardware level and summarize optimization targets from which. We divide preprocessing methods into three categories based on the optimization targets: preprocessing methods for efficient computing, efficient storage and efficient communication.

%---------------------------------------------------------------------------------------------------
%%%%% 本文使用的各种符号Notations
%---------------------------------------------------------------------------------------------------
\begin{table*}[h]
\vspace{-0.2cm}  %调整表格与上文距离
\caption{Notations and corresponding descriptions used in this paper}
\vspace{-0.3cm}  %调整表格标题距离
\begin{tabular}{cc}
\toprule
Notations                        & Descriptions                                        \\ 
\midrule
\textit{G}                       & A graph.                                            \\
\textit{V}, \textit{E}           & The vertex and edge sets of a graph.                \\
\textit{n}, \textit{m}           & The number of vertices and edges, \textit{n} = $\mid$\textit{V}$\mid$, \textit{m} = $\mid$\textit{E}$\mid$.  \\

\textit{v}                       & A vertex \textit{v} $\in$ \textit{V}.                \\
\textit{$e_{ij}$} $\in$ \textit{E}  & An edge from \textit{i} to \textit{j}.            \\
\textit{N}(\textit{v}), \textit{SN}(\textit{v})  & Original and sampled neighbourhood set of vertex \textit{v}.         \\

\textbf{A}, $\widetilde{\textbf{A}}$ & The original and normalized adjacency matrix of graph. \\
\textbf{D}, $\widetilde{\textbf{D}}$ & The degree matrix of \textbf{A} and $\widetilde{\textbf{A}}$.  \\
$\textbf{W}_{\textit{V}}$, $\textbf{W}_{\textit{E}}$   & The node and edge weight matrix of graph. \\
\textit{d} & The dimension of a vertex feature vector or hidden vertex feature vector.  \\
\textbf{X} $\in$ $\textbf{R}^{\textit{n$\times$d}}$   & The feature matrix of graph.    \\
$\textbf{x}_{\textit{v}}$ $\in$ $\textbf{R}^{\textit{d}}$   & The feature vector of the vertex \textit{v}, $\mid$$\textbf{x}_{\textit{v}}$$\mid$ = \textit{d}. \\

\textbf{x} $\in$ $\textbf{R}^{\textit{n}}$  & The feature vector of the vertex \textit{v} in the case of \textit{d} = 1. \\

\textbf{H}                       & The hidden feature matrix of graph.                  \\
$\textbf{h}_{\textit{v}}$ $\in$ $\textbf{R}^{\textit{d}}$ & The hidden feature vector of the vertex \textit{v}.  \\

\textit{L}                       & The number of GNN layers.                            \\
\textit{l}                       & The index of layer.                              \\
\textit{t}                       & The index of iteration.                          \\
$\sigma(\cdot)$                  & The nonlinear activation function.               \\
\bottomrule
\end{tabular}
\vspace{-0.2cm}  %调整表格与下文距离
\end{table*}

%---------------------------------------------------------------------------------------------------
%%%%% 图的表示和数据结构
%---------------------------------------------------------------------------------------------------
\subsection{Background of Graph Processing}
\textit{A. Graph Representation and Storage Format}
% 这里简单介绍不同存储格式的优缺点

A graph is represented as \textit{G} = (\textit{V}, \textit{E}), where the set of vertices \textit{V} = \{\textit{$v_{0}$},\textit{$v_{1}$},$\dots$,\textit{$v_{n-1}$}\}, and the set of edges \textit{E} = \{$\textit{$e_{0}$},\textit{$e_{1}$},$\dots$,\textit{$e_{m-1}$}$\}. $\textit{$v_{i}$}$ $\in$ $\textit{V}$ denotes a vertex in the graph, and $\textit{$e_{ij}$}$ = ($\textit{$v_{i}$}$, $\textit{$v_{j}$}$) $\in$ $\textbf{E}$ denotes an edge pointing from $\textit{$v_{i}$}$ (source) to $\textit{$v_{j}$}$ (destination). The vertex relationship is represented by an adjacency matrix \textbf{A} with size \textit{n$\times$n}. If \textit{$e_{ij}$} $\in$ \textit{E}, then \textit{$A_{ij}$} = 1, otherwise \textit{$A_{ij}$} = 0. The degree matrix \textbf{D} is a diagonal matrix, where \textit{$D_{ii}$} represents the degree of the vertex \textit{i}. The neighbourhood set of vertex \textit{v} is defined as \textit{N}(\textit{v}) = \{\textit{u} $\in$ \textit{V}$\mid$(\textit{v}, \textit{u}) $\in$ \textit{E}\}.


A graph may have vertex attributes represented as a multidimensional feature matrix \textbf{X} $\in$ $\textbf{R}^{\textit{n$\times$d}}$. $\textbf{x}_{\textit{v}}$ = ($\textit{$x_{0}$},\textit{$x_{1}$},$\dots$,\textit{$x_{d-1}$}$) is the feature vector of the vertex \textit{v} with dimension $\mid$$\textbf{x}_{\textit{v}}$$\mid$ = \textit{d}. $\textbf{W}_{\textit{V}}$ and $\textbf{W}_{\textit{E}}$ represent the vertex and edge feature matrix respectively. For GNN, $\textbf{h}_{\textit{v}}^{(\textit{l})}$ represents the hidden feature vector of layer \textit{l} of vertex \textit{v}, $\textbf{W}_{\textit{v}}^{(\textit{l})}$ and $\textbf{W}_{\textit{E}}^{(\textit{l})}$ represent the feature matrix of layer \textit{l}.

\begin{figure}[ht]
    \centering
    \vspace{-0.5cm}  %调整图片与上文的垂直距离
    \setlength{\abovecaptionskip}{-0.2cm}     %调整图片标题与图距离
    \setlength{\belowcaptionskip}{-0.2cm}   %调整图片标题与下文距离
    \includegraphics[width=1\textwidth]{fig-background/graph-representation.eps}
    \caption{Graph Representation and Storage Format}
    \label{fig:Representation}
\end{figure}

The adjacency matrix of a graph is generally a sparse matrix, and there are three main store formats of non-zero elements in the matrix: coordinate list (COO), compressed sparse row (CSR) and compressed sparse column (CSC). As shown in Figure \ref{fig:Representation}, the COO format stores row index, column index and value (features, weights, etc.) of non-zero elements in three arrays respectively. The COO format is simple and intuitive but contains many repeated elements, so CSR and CSC format are proposed to compress redundant data. The CSR format stores non-zero elements in three arrays with row compression. The first array is an offset array, which stores the offset position of the first non-zero element of each row in the column array. The last element of the offset array is the total number of non-zero elements in the matrix, so Offset\_Array\_Length = Row\_Number + 1. The second array sequentially stores the corresponding non-zero element column number, that is, the 1-hop destination vertex corresponding to an out-edge of source vertex in the row, so this array also called the edge array. The third array stores the value of each element. The CSC format is similar to CSR with column compression, and the edge array stores in-edges.

%---------------------------------------------------------------------------------------------------
%%%%% 图的特点
%---------------------------------------------------------------------------------------------------
\noindent{\textit{B. Graph Processing Characteristics}}

Graphs in real-world are often extremely large. User network graph of twitter in 2012 has had 175 million active users with about 20 billion edges\cite{2014Twitter}. Facebook's social network graph in 2015 has already contained more than 2 billion vertices and more than a trillion edges\cite{2015facebook}. In addition to the number of edges and vertices, the feature vector dimension representing the attributes in real graphs exceeds thousands, which further expands the data scale of graphs.

The graph structure has three characteristics: \textit{un-structure}, \textit{sparsity}, and \textit{power-law distribution}. Because the relationship between objects in real life is often uncertain, the structure of the graph is usually not fixed. For most objects have no connections, most graphs are extremely sparse\cite{2019alleviating}. Since the degree of different vertices is not even, the graph presents a power-law distribution characteristic\cite{2012powergraph}, that is, a few vertices are connected to a large number of vertices, and most vertices are connected to a small number of vertices. For example, in a social network, a few celebrities are followed by most people, while most ordinary users are barely followed.

%---------------------------------------------------------------------------------------------------
%%%%% 现有的图算法和通用编成模型
%---------------------------------------------------------------------------------------------------
\noindent{\textit{C. Graph Processing Algorithms}}

Graph processing applications mainly include traditional graph processing applications and graph neural network (GNN) applications.

%------------------ 传统图计算 ------------------
\textbf{Traditional Graph Applications}: The main programming models of traditional graph processing applications include vertex-centric programming model(VCPM)\cite{2010Pregel} and edge-centric programming model(ECPM)\cite{2013X-stream}, both of which can be abstracted by the GAS model(Gather, Apply, Scatter)\cite{2012powergraph}. The Gather stage collects the neighbor information of in-edges, the Apply stage updates the attribute information of the center vertex according to the collected information, and the Scatter stage updates the neighbor vertex information of out-edges using the new value. The three stages execute iteratively until the number of iterations hits the ceiling or the results are completely converged. The three stages execute iteratively until the number of iterations hits the ceiling or the results are converged. As shown in Figure \ref{fig:VCPM_ECPM}, the VCPM gathers the neighbour information of each activation vertex, then passes information to the neighbor vertices. The ECPM collects the source vertices' information of each edge and updates the destination vertex accordingly.

\begin{figure}[ht]
    \centering
    \vspace{-0.5cm}  %调整图片与上文的垂直距离
    \setlength{\abovecaptionskip}{-0.2cm}     %调整图片标题与图距离
    \setlength{\belowcaptionskip}{-0.5cm}   %调整图片标题与下文距离
    \includegraphics[width=1\textwidth]{fig-background/VCPM_ECPM.eps}
    \caption{Scatter-Gather stage of programming model\cite{2013X-stream}}
    \label{fig:VCPM_ECPM}
\end{figure}

Traditional graph processing algorithms are roughly divided into two categories: Stationary Graph Algorithms and Non-stationary Graph Algorithms\cite{2013Mizan}. The stationary graph algorithms update all vertices per iteration and typical algorithms are PageRank (PR), Diameter Estimation, etc. The non-stationary graph algorithms update neighbours from the activation vertices, and typical algorithms are Breadth First search (BFS), Single Source Shortest Path (SSSP), etc. Table \ref{table:VCPM-Alg} shows the algorithms implement in vertex-centric model\cite{2019alleviating}. The VCPM can be expressed as three functions: \textit{Process\_Edge}, \textit{Reduce} and \textit{Apply}. Take PR for example: First, function Process\_edge gains the value of each source vertex's property which is the edge processing result. Second, the result is sent to function Reduce, and the reduction operation (summation) is performed with the temporary vertex property. Third, after finishing all edge traversal, function Apply updates the destination vertex property using the temporary property and constant coefficient.

\begin{table*}[h]
\vspace{-0.15cm}  %调整表格与上文距离
\caption{Algorithm Implement in Vertex-centric Model}
\vspace{-0.3cm}  %调整表格标题距离
\label{table:VCPM-Alg}
\begin{threeparttable}
\renewcommand{\arraystretch}{1}%调行距
\setlength\tabcolsep{20pt}%调列距
\begin{tabular}{cccc}
\toprule
Algorithm       & \textit{Process\_Edge}                             & \textit{Reduce}                                   & \textit{Apply}                                               \\ 
\midrule
PR              & \textit{v.Prop}                                    & \textit{v.tProp} + \textit{res}                   & ($\alpha$ + $\beta$ $\cdot$ \textit{u.tProp})/\textit{u.deg} \\
BFS             & \textit{v.Prop} + 1                                & \textit{min} (\textit{u.tProp}, \textit{res})     & \textit{min} (\textit{u.Prop}, \textit{u.tProp})              \\
SSSP            & \textit{min}(\textit{v.tProp}, \textit{e.weight})  & \textit{max} (\textit{u.tProp}, \textit{res})     & \textit{max} (\textit{u.Prop}, \textit{u.tProp})              \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\footnotesize
\item Note: The edge is \textit{e}(\textit{v}, \textit{u}). The \textit{res} and \textit{u.deg} represent edgeProResult and \textit{u.cProp} respetively. The $\alpha$ and $\beta$ are constant coefficient.
\end{tablenotes}
\end{threeparttable}
\vspace{-0.15cm}  %调整表格与下文距离
\end{table*}

%------------------ 图神经网络 ------------------
\textbf{Graph Neural Network Applications}: Graph neural network combines graph structure and neural networks (NN). Similar to neural network, a complete graph neural network includes two main parts: train and inference. The train process adjusts the loss function with back-propagation, improving the model prediction accuracy by reducing the gradient of the loss function. Inference process uses the trained model to make predictions. The mains graph neural network algorithms can be abstracted into the following model:

\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\textbf{h}_{\textit{N}(\textit{v})}^{(\textit{l})} = \textbf{Aggregate}^{(\textit{l})}(\{ \textbf{h}_{\textit{u}}^{(\textit{l-1})} : \textit{u} \in \textit{N}(\textit{v}) \})
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}

\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\textbf{h}_{\textit{v}}^{(\textit{l})} = \textbf{Update}^{(\textit{l})}(\{\textbf{h}_{\textit{v}}^{(\textit{l-1})}, \textbf{h}_{\textit{N}(\textit{v})}^{(\textit{l})}\})
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}

\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
%\textbf{\textit{Loss}}
minimize:  \mathcal{L}( \{\textbf{h}_{\textit{v}}^{\textit{(L)}} | \textit{v} \in \textit{V}\})
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}

In aggregrate stage, the graph neural network traverses the entire graph to aggregate the neighbor information for each vertex, obtaining the aggregated intermediate feature of this layer ($\textbf{h}_{\textit{N(v)}}^{\textit{(l)}}$). In Update stage, the intermediate feature of this layer ($\textbf{h}_{\textit{N(v)}}^{\textit{(l)}}$) and the output feature of previous layer ($\textbf{h}_{\textit{v}}^{\textit{(l-1)}}$) are combined to update the output feature vector of this layer ($\textbf{h}_{\textit{v}}^{\textit{(l)}}$). The aggregation stage usually performs operations such as accumulation, mean, maximum (max), minimum (min), pooling, etc. The Update stage usually inplemented by multi-layer perceptron (MLP), gated recurrent unit (gated recurrent GRU), nonlinear activation function, etc. 

For a variety of scenario needs, many variants of GNN are proposed, such as graph convolution network (GCN), graph attention network (GAT), recurrent graph neural network (RGNN), and graph auto-encoders (GAE)\cite{qinghua2020comprehensive}. Then, we take GCN as an example for formulaic introduction\cite{2017GCN}:

\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:GCN}
\textbf{H}^{\textit{l}} = \sigma \left( \widetilde{\textbf{D}}^{-\frac{1}{2}}\widetilde{\textbf{A}}\widetilde{\textbf{D}}^{-\frac{1}{2}}\textbf{H}^{\textit{l}-1}\textbf{W}^{\textit{l}-1} \right)
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}

The forward propagation of GCN is iteratively computed in a layer manner. Given the input layer \textbf{H}(0)=\textbf{X}, the output layer \textbf{H}(L)=\textbf{Z}, the hidden layer of GCN is expressed as the Equation \ref{equation:GCN}, where \textbf{W} is the trainable weight matrix. The back propagation uses the stochastic gradient descent method to update the gradient, and then adjust the training parameter matrix W.

%---------------------------------------------------------------------------------------------------
%%%%% 现有预处理方法：sampling，sparsification, partition, quantization, reconstruction, blocking
%---------------------------------------------------------------------------------------------------
\subsection{Graph Preprocessing Methods}

% 如表x所示，现有的图预处理方法按照核心机制可以分为七种主要类型。 其中，分区, 采样、稀疏化和重构改变了图的表示，而量化、重排序和重排在不改变图结构的情况下改变了数据的表示。 下面分别介绍这几种预处理方法的基本原理。
As shown in Table \ref{table:preprocessing-method}, the existing graph preprocessing methods can be divided into seven main types according to the core mechanism. Among them, partition, sampling, sparsification and reconstruction change the graph representation, while quantization, reorder, and blocking change the data representation without changing graph structure. Next we will introduce the fundamental of these preprocessing methods respectively.

\begin{table*}[h]
\vspace{-0.15cm}  %调整表格与上文距离
\caption{Existing graph preprocessing methods}
\vspace{-0.3cm}  %调整表格标题距离
\label{table:preprocessing-method}
%\renewcommand{\arraystretch}{1.2}%调行距
%\setlength\tabcolsep{10pt}%调列距
\begin{tabular}{|l|l|l|}
\hline
\textbf{Mechanism} & \textbf{Method} & \textbf{Works}    \\
\hline
\multirow{4}{*}{\makecell[l]{Graph\\Representation\\Change}}
& \makecell{\textcircled{a}\\Partition} & \makecell[l]{
                Vertex Partition: METIS \cite{1998METIS}\cite{2020DistDGL}, RandomHash \cite{2012graphlab}\cite{2010Pregel}, LDG\cite{2012LDG}\cite{2020PaGraph} \\
                Edge Partition: PowerGraph \cite{2012powergraph}, BalanceEdge \cite{2014BalanceEdgePartition}, DBH \cite{2014DBH}, NE \cite{2017NE} \\
                Others: GAP \cite{2019GAP}, PowerLyra \cite{2019powerlyra} }\\
\cline{2-3}
& \makecell{\textcircled{b}\\Sampling}  & \makecell[l]{
                Node-wise Sampling: GraphSAGE \cite{2017graphsage}, PinSage \cite{2018PinSage}, SSE \cite{2018SSE}, VR-GCN \cite{2019VR-GCN} \\
                Layer-wise Sampling: FastGCN \cite{2018FastGCN}, AS-GCN \cite{2021AS-GCN}, LADIES\cite{2019LADIES}  \\
                Subgraph-based Sampling: Cluster-GCN \cite{2019Cluster-GCN}, GraphSAINT \cite{2019graphsaint}, RWT \cite{2021RWT} \\
                Heterogeneous Sampling: HetGNN \cite{2019HetGNN}, HGSampling \cite{2020HGSampling}} \\                
\cline{2-3}
& \makecell{\textcircled{c}\\Sparsification}   & \makecell[l]{
                Heuristic Sparsification: DropEdge \cite{2020DropEdge}, FastGAT \cite{2020FastGAT}, DyGNN \cite{2021DyGNN} \\
                Learnable module for Sparsification: NeuralSparse \cite{2020NeuralSparse}, SGCN \cite{2020SGCN}, GAUG \cite{2021GAUG}, \\
                GLT \cite{2021GLT}, AdaptiveGCN \cite{2021Adaptivegcn}} \\
\cline{2-3}
& \makecell{\textcircled{d}\\Reconstruction} &  
                GraphACT \cite{2020GraphACT}, work \cite{2020GcnInference}, Redundancyfree \cite{2020Redundancy-free}, I-GCN \cite{2021I-gcn}   \\
\hline
\multirow{3}{*}{\makecell[l]{Data\\Representation\\ Change}}
& \makecell{\textcircled{e}\\Quantization} & \makecell[l]{
                Degree-free Quantization: Bi-GCN \cite{2021Bi-GCN}, DCGNN \cite{2021DCGNN}, EXACT \cite{2021EXACT} \\
                Degree-based Quantization: DegreeQuant\cite{2020DegreeQuant}, DBQ\cite{2022DBQ}, SGQuant \cite{2020SGQuant} } \\
\cline{2-3}
& \makecell{\textcircled{f}\\Reorder}  &  \makecell[l]{
                Heavyweight Reorder: Gorder \cite{2016Gorder}, Recall \cite{2017Recall} \\
                Lightweight Reorder: RCM \cite{1984RCM}\cite{2014ParallelRCM}\cite{2017RCM}\cite{2020GcnInference}, FBC \cite{2017Cagra}, ReorderHC \cite{2018ReorderHC}, DBG \cite{2019DBGreorder},\\ reorder-in-GNN \cite{2021rubik}\cite{2022H-GCN}\cite{2022GCoD}} \\
\cline{2-3}
& \makecell{\textcircled{g}\\Blocking}  & \makecell[l]{
                Shard-split: Graphchi \cite{2012graphchi}, TurboGraph \cite{2013TurboGraph}, FPGP \cite{2016fpgp}, HyGCN \cite{2020HyGCN} \\
                Loop-tiling: AWB-GCN \cite{2020awbgcn}, EnGN \cite{2020EnGN}, GCNAX \cite{2021GCNAX}, SnF \cite{2022SnF}}  \\
\hline
\end{tabular}
\vspace{-0.15cm}  %调整表格与下文距离
\end{table*}

%%%%%%------------------------------------ graph representation ----------------------------------------
\noindent{\textit{A. Methods of changing graph representation}}

%% 图片 Graph-structure：Sample, Sparsification, Partition, reconstruction
\begin{figure}[ht]
    \centering
    \vspace{-0.2cm}  %调整图片与上文的垂直距离
    \setlength{\abovecaptionskip}{0.cm}     %调整图片标题与图距离
    \setlength{\belowcaptionskip}{-0.2cm}   %调整图片标题与下文距离
    \includegraphics[width=\textwidth]{fig-background/graph-method.eps}
    \caption{Methods of changing Graph-representation : (a) Partition method; (b) Sampling method; (c) Sparsification method; (d) Reconstruction method}
    \label{fig:graph-method}
\end{figure}

%-------- parititon ----------
\textcircled{a} \textbf{Partition}

%大规模图处理很难在单台机器上有效执行。 一种常见的解决方案是将图数据分发到多个节点进行计算[]。 图划分是将原始图划分为多个子图，分配给多个节点进行计算的过程。 图 x(a) 是图划分的一个示例，其中使用顶点切割策略将原始图划分为3个互斥的子图。 图分区有两个目的：一是尽可能将顶点和边均匀分布到不同节点，实现负载均衡； 二是可以通过分区来改善数据局部性，以减少节点之间的通信开销。图划分在传统图计算和图神经网络中都得到广泛应用。
Large scale graph processing is difficult to perform effectively on a single machine. A common solution is to distribute graph data to multiple nodes for computing \cite{2012StreamingPartition}. Graph partition is the process of dividing original graph into multiple subgraphs and assigning them to multiple nodes for computing. Figure \ref{fig:graph-method} (a) is an example of graph partition, where the original graph is divided into 3 mutually exclusive subgraphs using vertex-cut strategy. Graph partition has been an NP-hard problem \cite{2016RecentPart} serving two goals: One is that vertices are evenly distributed to different nodes to extent possible, achieving load balance; Two is that edge-cut is minimized to to reduce communication overhead between nodes. Graph partition is widely used in both traditional graph computing and graph neural networks. We generally formulate the process of graph partition as follows:

\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:partition_1}
%{\rm Partition}
\textbf{Partition}(\textit{V})= \{{\bigcup}_{i} \textit{V}_\textit{i} \vert i=1,\cdots,\textit{k}; \forall i \neq j, \textit{V}_\textit{i} \cap \textit{V}_\textit{j} = \emptyset, \}% \textit{V}_1 \cup \textit{V}_2 \cdots \cup \textit{V}_\textit{k} \{\textit{V}_\textit{i} \cap \textit{V}_\textit{j} = \emptyset, \forall i \neq j\}
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}

\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:partition_2}
\{Block_i \vert i=1,\cdots,k\} = \textbf{LoadBalance}(V_i, \cdots, V_k) %{\rm LoadBalance}(V_i, \cdots, V_k)
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}

\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:partition_3}
\{Subgraph_i \vert i=1,\cdots,k\} = \textbf{MinEdgeCut}(E, \{Block_i \vert i=1,\cdots,k\}) %{\rm MinEdgeCut}(E, \{Block_i \vert i=1,\cdots,k\})
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}

%图的划分方法根据划分方式[BalanceEdge]可分为两种：顶点划分（edge-cut）和边划分（vertex-cut）。 顶点划分将顶点分配到不同的子图中，使得跨越不同子图的边被分割（切边）。RandomHash[Pregel][graphlab]、METIS[]、LDG[]都是经典的顶点划分方法。 对于幂律图，有些顶点的边太多，采用点划分可能会造成大量的边缺失，而边分区则可以更好的处理这些问题。边分区将边分配给不同的子图，其中一些顶点被复制并分布在不同的子图中（图 x(c)）。 PowerGraph[]、balanceEdge[]、DBH[]、NE[]、GAP[]等是经典的边划分方法。对于稠密图，边划分会导致大量顶点复制，需要更大的缓存空间。为了实现更好的划分，一些新的图划分方法被提出。GAP[]使用神经网络进行图划分，PowerLyra[]基于顶点的度有选择的使用点划分和边划分。
Graph partition methods can be divided into two types according to the partition way \cite{2014BalanceEdgePartition}: vertex partition (edge-cut) and edge partition (vertex-cut). Vertex partition assigns vertices into different subgraphs, so that edges crossing different subgraphs are split (edge-cut). METIS \cite{1998METIS}\cite{2020PCGCN}\cite{2020DistDGL}, RandomHash \cite{2012graphlab}\cite{2010Pregel}, LDG \cite{2012LDG}\cite{2020PaGraph} are classic vertex partition methods. For power-law graphs, some vertices have too many edges, which vertex partition may cause a large number of edge-missing, while edge partition can better deal with the problem. Edge partition assigns edges to different subgraphs with some vertices being replicated and distributed in different subgraphs (Figure \ref{fig:graph-method} (c)). PowerGraph \cite{2012powergraph}, BalanceEdge \cite{2014BalanceEdgePartition}, DBH \cite{2014DBH}, NE \cite{2017NE} use edge partition method. For dense graphs, edge partition leads to a large number of vertex duplication, requiring larger cache space. To achieve better partition, some new graph partitioning methods are proposed. GAP \cite{2019GAP} uses neural networks to divide graphs, PowerLyra \cite{2019powerlyra} selectively uses vertex partition and edge partition based on the degree of vertices.

%-------- sampling ----------
\textcircled{b} \textbf{Sampling}

%使用full-batch的卷积神经网络训练存在两个问题：首先，每一层都要遍历整个图，因此很难将大图的所有顶点存储在内存中。 其次，全批训练每个 epcoh 更新一次，导致收敛速度非常慢。 使用 mini-batch 训练可以解决这两个问题：对于第一个问题，它每次加载一个 mini-bach 数量的顶点而不是整个图，这有效地缓解了内存压力。 对于第二个问题，每次迭代更新一次，加快了收敛速度。 采样是通过选择顶点创建小批量的过程，与全批量训练相比，它减少了计算和存储开销。 图 x(b) 是图抽样的示例，其中选择顶点的部分 2 跳邻居来为后续训练创建小批量。 图采样的过程表述如下：
There are two problems in the convolutional neural network training using full-batch: First, the entire graph is traversed in each layer, so it is difficult to store the whole vertices of a large graph in memory. Second, full-batch training updates once per epcoh, leading to very slow convergence. Training with mini-batch can solve these two problems: For the first problem, it loads a mini-bach number of vertices instead of the whole graph each time, which effectively relieves memory pressure. For the second problem, each iteration is updated once, which speeds up the convergence speed. Sampling is the process of creating mini-batches by selecting vertices, which reduces computing and storage overhead compared to full-batch training. Figure \ref{fig:graph-method} (b) is an example of graph sampling, where part of the 2-hop neighbors of vertices are selected to create mini-batches for subsequent training. The process of graph sampling is formulated as follows:

\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:sample_1}
SN (v) = \textbf{Sampling}^{(l)}(N(v))
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}

\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:sample_2}
\textbf{h}_{\textit{N}(\textit{v})}^{(\textit{l})} = \textbf{Aggregate}^{(\textit{l})}(\{ \textbf{h}_{\textit{u}}^{(\textit{l-1})} : \textit{u} \in \textit{SN}(\textit{v}) \})
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}

\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:sample_3}
\textbf{h}_{\textit{v}}^{(\textit{l})} = \textbf{Update}^{(\textit{l})}(\{\textbf{h}_{\textit{v}}^{(\textit{l-1})}, \textbf{h}_{\textit{N}(\textit{v})}^{(\textit{l})}\})
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}

%根据顶点选择方式[]，图采样方法可分为四种类型：节点采样、层采样、基于子图的采样和异构采样。 node-wise sampling方法选择顶点的邻居作为子图，GraphSage[]、PinSage[]、SSE[]和VR-GCN[]是经典的node-wise采样模型。 尽管逐节点采样限制了每个顶点的邻居数量，但邻居总数随着层数的增加呈指数级增长。 为了控制顶点的数量，逐层采样方法在每一层中采样固定数量的顶点。然而，随着层数的加深，子图变得越来越稀疏。经典的 layer-wsie 采样包括 FastGCN[]、AS-GCN[]、LADIES[]。基于子图的采样选择一个或多个顶点作为初始顶点，然后按照特定的策略对节点和边集进行采样，具有较好的独立性。 基于子图的采样工作有Cluster-GCN[]、GraphSAINT[]、RWT[]等。异构采样用于处理异构图，解决邻居数量和类型不平衡的问题。 异构作品包括 HetGNN[] 和 HGSampling[]。
Graph sampling methods can be divided into four types according to the vertex selecting way\cite{2021liu-sampling-survey}: node-wise sampling, layer-wise sampling, subgraph-based sampling, and heterogeneous sampling. The node-wise sampling method selects the neighbors of vertices as subgraphs, GraphSage\cite{2017graphsage}, PinSage\cite{2018PinSage}, SSE\cite{2018SSE}, and VR-GCN\cite{2019VR-GCN} are classic node-wise sampling models. Though node-wise sampling limits the neighbor number of each vertex, the total number of neighbors explodes exponentially with the number of layers increasing. To control the number of vertices, layer-wise sampling method samples a fixed number of vertices in each layer. However, the subgraphs become sparser with the number of layers deepening. Classic layer-wsie sampling includes FastGCN\cite{2018FastGCN}, AS-GCN\cite{2021AS-GCN}, and LADIES\cite{2019LADIES}. Subgraph-based sampling selects one or more vertices as initial vertices, and then samples vertex and edge sets according to a specific strategy, which has better independence. Subgraph-based sampling works include Cluster-GCN\cite{2019Cluster-GCN}, GraphSAINT\cite{2019graphsaint}, RWT\cite{2021RWT}, etc. Heterogeneous sampling is used to deal with heterogeneous graphs, solving the problem of imbalance neighbor number and types. Heterogeneous works include HetGNN\cite{2019HetGNN} and HGSampling\cite{2020HGSampling}.

%-------- Sparsification ----------
\textcircled{c} \textbf{Sparsification}

%大规模图神经网络具有海量的特征和权重数据，导致计算和存储开销大。 事实上，在计算过程中存在大量冗余数据，剔除不影响精度。 稀疏化[1997]是一种经典的冗余消除技术，广泛用于动态图加速。 它删除了图不必要的边，同时保留了输入图的尽可能多的信息。 与任务无关的边称为冗余边，可以去掉冗余边以减少冗余计算，减轻存储压力。 此外，稀疏化有助于增加计算的随机性，从而缓解训练的过度平滑问题。 图 x(c) 是图稀疏化的示例，其中删除了一些边。 图稀疏化的过程表述如下：
Large-scale graph neural networks have massive data of feature and weight, resulting in large computing and storage overhead. In fact, there are a lot of redundant data in the computing process, removing which do not affect the accuracy. Sparsification\cite{sparsification1997} is a classic redundancy elimination technique which is widely used for dynamic graph acceleration. It removes unnecessary edges for the graph while retaining as much information as possible of the input graph. Edges that are irrelevant to tasks are called redundant edges, which can be removed to reduce redundant computing and relieve storage pressure. In addition, sparsification helps to increase the randomness of the computing, thereby alleviating the over-smoothing problem of training. Figure \ref{fig:graph-method} (c) is an example of graph sparsification, where some edges are removed. The process of graph sparsification is formulated as follows:

\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:sparse_1}
\textbf{A}_{sp} = Sparse(\textbf{A}) = \begin{cases} \textbf{Heuristic.Algo}(\textbf{A}) &\\ \textbf{Sparsifier}(\textbf{A}) \end{cases}
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}

\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:sparse_2}
GNN(\textbf{A}_{sp}) \rightarrow Training\ \&\ Inference
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}

%稀疏化方法根据丢弃策略可分为两类：启发式稀疏化和用于稀疏化的可学习模块。 对于启发式稀疏化，丢弃边的策略是启发式的，不考虑全局优化目标。 DropEdge[]、FastGAT[]、DyGNN[] 是典型的启发式作品。 用于稀疏化的可学习模块通常构建一个稀疏化器作为优化目标。 NeuralSparse[]、SGCN[]、GAUG[]、GLT[]、AdaptiveGCN[]等作品都采用了这种策略。
Sparsification methods can be divided into two types according to the dropping strategy\cite{liu2022survey}: heuristic sparsification and learnable module for sparsification. For Heuristic sparsification, the strategy of discarding edges is heuristic which does not consider the global optimization target. DropEdge \cite{2020DropEdge}, FastGAT \cite{2020FastGAT}, and DyGNN \cite{2021DyGNN} are typical heruistic works. The learnable module for sparsification generally builds a sparsifier as an optimization target. NeuralSparse \cite{2020NeuralSparse}, SGCN \cite{2020SGCN}, GAUG \cite{2021GAUG}, GLT \cite{2021GLT}, AdaptiveGCN\cite{2021Adaptivegcn} and other works all use this strategy.

%-------- Reconstruction ----------
\textcircled{d} \textbf{Reconstruction}

%复杂图中有很多共享邻居，这意味着图算法执行过程中会发生大量的重复计算。 合并共享邻居是减少重复计算的有效方法，称为图重构。 一方面，使用重构图可以有效减少重复操作，提高计算效率。 另一方面，图重构可以提高数据重用率，减少不必要的片外内存访问。如图 x(d) 所示，共享顶点合并为顶点簇，在执行算法时将其作为一个整体而不是单独的顶点进行计算。图重构的过程表述如下：
There are many shared neighbors in complex graphs, which means a large number of repetitive computing occur in graph algorithms execution. Merging shared neighbors is an effective way to reduce double computing, which is called graph reconstruction. On the one hand, using reconstructed graph can effectively reduce repetitive operations, improving computing efficiency. On the other hand, graph reconstruction can improve data reuse rate, reducing unnecessary off-chip memory access. As shown in Figure \ref{fig:graph-method} (d), shared vertices are merged into vertex clusters, which are computed as a whole rather than separate vertices when executing algorithms. The process of graph reconstruction is formulated as follows:

\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:reconstruction_1}
Construction(\textbf{G}_{s}) = \begin{cases} \textbf{CommonPairsMatching}(\textbf{M}_{a}) &\\ \textbf{Update}(\textbf{G}_{a}, \textbf{M}_{a}) \end{cases}
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}

\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:reconstruction_2}
\textbf{G}_{s} \rightarrow Aggregation
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}

%图重构方法已在多项工作中得到使用。 GraphACT[]和work[hardware acc]通过预处理合并共享邻居，消除了邻居顶点的冗余归约操作。 Work [redundancy-free] 提出了 Hierarchically Aggregated computation Graphs (HAGs)，它合并了可以重复使用的中间结果，去除了 GNN 训练中的重复计算和冗余数据移动。 I-GCN【】也使用了重构方法来合并公共邻居。与稀疏化方法不同，图重构方法只预先计算部分数据，几乎不会造成信息丢弃。
Graph reconstruction methods have been applied in several works. GraphACT \cite{2020GraphACT} and work \cite{2020GcnInference} combine shared neighbors through preprocessing, eliminating redundant reduction operations of neighbor vertices. Redundancyfree\cite{2020Redundancy-free} proposes Hierarchically Aggregated computation Graphs (HAGs), which merges intermediate results which can be reused, removing repetitive computing and redundant data movement in GNN training. I-GCN \cite{2021I-gcn} combines common neighbours through reconstruction. Different from the sparsification method, graph reconstruction method only computes part data in advance, which hardly causes information discarding.

%%%%%%-------------------------------------- data structure ------------------------------------------
\noindent{\textit{B. Methods of changing data representation}}

%% 图片：Data-structure：Quantization, Reorder, blocking
\begin{figure}[ht]
    \centering
    \vspace{-0.2cm}  %调整图片与上文的垂直距离
    \setlength{\abovecaptionskip}{0.cm}     %调整图片标题与图距离
    \setlength{\belowcaptionskip}{-0.8 cm}   %调整图片标题与下文距离
    \includegraphics[width=\textwidth]{fig-background/data-method.eps}
    \caption{Methods of changing data-representation : (a) Quantization method; (b) Reorder method; (c) Blocking method}
    \label{fig:data-method}
\end{figure}

%-------- Quantization ----------
\textcircled{e} \textbf{Quantization}

%GNN 将神经网络扩展到了图应用。 与传统的图算法不同，图神经网络具有高维特征向量，这带来了巨大的计算和内存访问开销。 模型量化是减少数据量的有效方法，其核心思想是神经网络是鲁棒的，因此降低模型精度只是损失了噪声。 量化是指将连续的浮点值数据转换为有限位数的离散值的过程\cite{2022DBQ}。 离散值的类型为整型，如图x(a)所示，将32bit的浮点数量化为2bit的整数，大大减少了存储开销。
GNN has extended neural networks to graph applications. Unlike traditional graph algorithms, graph neural networks have high dimensional feature vectors, which brings huge computing and memory access overhead. Model quantization is an effective way to reduce data amount, whose core idea is the neural network is robust, so reduce model accuracy only losses noise. Quantization refers to the process of converting continuous floating-point value data into discrete values with a limited number of bits\cite{2022DBQ}. The type of discrete value is integer type, as shown in Figure \ref{fig:data-method} (a), 32bit floating point number is quantified into 2bit integer number, which greatly reduce storage overhead. The process of graph quantization is formulated as follows:

\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:quant_1}
\textbf{G}_{quantized} = \textbf{Quant}(\textbf{G}) \rightarrow Forward
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}

\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:quant_2}
\textbf{G}_{dequantized} = \textbf{Dequant}(\textbf{G}_{quantized}) \rightarrow Backward
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}

%图量化大致可以分为两种类型：无度量化和基于度的量化。 无度量化策略不考虑顶点度，这些工作大多直接将经典的 CNNs 量化方法扩展到 GNNs。 DCGNN [2021DCGNN] 和 Bi-GCN [Bi-GCN] 将二值化策略引入 GNN。 EXACT[] 使用压缩激活来训练 GNN。 与 CNN 相比，GNN 模型具有非均匀拓扑结构，因此一些方法基于顶点的度数进行量化。 DegreeQuant [DegreeQuant] 和 DBQ [DBQ] 使用基于度的量化方法，而 SGQuant[] 执行基于多粒度的量化。 这些量化方法可以更好地减少量化精度的损失。
Graph quantization can be roughly divided into two types: degree-free quantization and degree-based quantization. The degree-free quantization strategy do not considers the vertex degree, and most of these works directly extend the classical CNNs quantization method to GNNs. DGCNN \cite{2021DCGNN} and Bi-GCN \cite{2021Bi-GCN} introduce binarization strategies to GNNs. EXACT[] uses compressed activations to train GNNs. Compared with CNNs, GNN models have a non-uniform topology, so some methods quantify based on the degree of vertices. DegreeQuant \cite{2020DegreeQuant} and DBQ \cite{2022DBQ} use degree-based quantization methods, and SGQuant \cite{2020SGQuant} performs quantization based on multiple granularities. These quantization methods can better reduce the loss of quantization accuracy.

%-------- Reorder ----------
\textcircled{f} \textbf{Reorder}

%图结构的不规则性导致图算法执行过程中存在大量不规则访问，内存访问的时空局部性较差。 通过顶点重新排序的提前数据布局优化是一种广泛使用的技术，用于改善图形分析中的内存访问局部性。 图重排方法是通过重新标记每个顶点的ID来实现的。 如图x(b)所示，具有原始ID的邻接矩阵中的数据是分散的，重新排序的邻接矩阵中的数据具有更好的局部性。 Reorder技术可以有效减少不规则的内存访问，提高带宽利用率。
The irregularity of graph structure results in a large number of irregular access in executing graph algorithms, which takes poor temporal and spatial locality of memory accesses. Ahead data layout optimization via vertex reordering is a widely used technique to improve memory access locality in graph analysis. The graph blocking method is realized by relabeling the ID of each vertex. As shown in Figure \ref{fig:data-method} (b), data in adjacency matrix with original IDs is scattered and data in reordered adjacency matrix has better locality. Reorder technology can effecively reduce irregular memory access and improve bandwidth utilization. The process of reorder is formulated as follows:

\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:reorder_1}
\textbf{A}_{r} = \textbf{Reorder}(\textbf{A})
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}

\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:reorder_2} 
\textbf{A}_{r} \rightarrow \begin{cases} \textbf{Scatter} \quad Traditional &\\ \textbf{Aggregate} \quad GNN \end{cases}
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}

%早期的重排序算法如 Gorder [2016Gorder] 和 Recall [2017Recall] 是重量级算法，通过数据重排序提供显着的性能提升，但计算复杂度高。 RCM[1984RCM][2014ParallelRCM][2017RCM][2020GcnInference] 、FBC[2017Cagra]、ReorderHC[2018ReorderHC]、DBG[2019DBGreorder] 等轻量级重排序算法减少了重排序时间，更适合在线预处理。 Rubik[2021Rubik]、H-GCN[H-GCN],GCoD[]在 GNN 中使用了轻量的重新排序技术，利用片上数据的可重用性来提高缓存效率。
Earlier reorder algorithms such as Gorder \cite{2016Gorder} and Recall \cite{2017Recall} are heavyweight algorithms, which provide significant performance improvement through data reorder, but have high the computational complexity. Lightweight reorder algorithms such as RCM 
 \cite{1984RCM}\cite{2014ParallelRCM}\cite{2017RCM}\cite{2020GcnInference}, FBC \cite{2017Cagra}, ReorderHC \cite{2018ReorderHC} and DBG \cite{2019DBGreorder} reduce the reorder time and is more suitable for online preprocessing. Rubik \cite{2021rubik}, H-GCN \cite{2022H-GCN}, GCoD \cite{2022GCoD} use reorder technology in GNNs, exploiting the reusability of on-chip data to improve cache efficiency. 

%--------blocking ----------
\textcircled{g} \textbf{Blocking}

% 大规模图处理很难将所有数据都缓存在芯片上，因此需要片外数据移动。 图的不规则结构导致不规则的内存访问模式，导致大量随机内存访问，严重限制了整体性能。 blocking通过数据布局优化改进数据流访问形式，从而增加数据的可重用性并提高存储带宽利用率。 图 x(c) 显示了基于列的矩阵乘法分块，其中向量可以在分块后多次重复使用。 分块过程描述如下：
Large-scale graph processing is difficult to cache all data on the chip, so it requires off-chip data movement. The irregular structure of the graph leads to irregular memory access patterns, resulting in large number of random memory accesses which severely limits the overall performance. Blocking improves data flow access form through data layout optimization, which increases data reusability and improves storage bandwidth utilization. Figure \ref{fig:data-method} (c) shows column-based matrix multiplication blocking, where the vector can be reused multiple times after blocking. The blocking process is described as follows:

\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:blocking_2} 
\textbf{G} \rightarrow \textbf{Blocking}(\textbf{G}) \rightarrow \begin{cases} \textbf{Scatter} \quad Traditional &\\ \textbf{Aggregate} \quad GNN \end{cases}
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}

%常用的分块方法可以分为两种：shard-split方法和loop-tiling方法。 Shard-split方法将图数据划分为区间和分片，每个区间内的顶点编号是连续的，从而实现连续的数据访问。 循环平铺方法用于优化稀疏矩阵乘法运算[自适应]。 这种方法扩展到GCNs，将GCNs分成多个tiling，然后通过限制计算范围来提高缓存效率。 shard-split方法主要用在传统的图计算框架中，典型的工作有graphchi[]、Turbograph[]、FPGP[]。 此外，HyGCN[] 使用 shard-split 来加速 GCN 推理。 采用loop-tiling方法加速GCNs，典型工作有AWB-GCN【】、EnGN、GCNAX【】、SnF【】。
Common blocking methods can be divided into two types: shard-split method and loop-tiling method. Shard-split method divides graph data into intervals and shards, in which the vertex numbers in each interval are continuous, thereby realizing continuous data access. The loop-tiling methods are used to optimize sparse matrix multiplication operation \cite{2019AdaptiveTilingSpMM}. This method is extended to GCNs, which divides GCNs into multiple tilings, and then improve cache efficiency by limiting the calculation range. The shard-split method is mainly used in the traditional graph computing framework, and the typical work is graphchi \cite{2012graphchi}, Turbograph \cite{2013TurboGraph}, and FPGP \cite{2016fpgp}. Besides, HyGCN \cite{2020HyGCN} uses shard-split to speed up GCN inference. The loop-tiling method is used to accelerate GCNs, and the typical work is AWB-GCN \cite{2020awbgcn}, EnGN \cite{2020EnGN}, GCNAX \cite{2021GCNAX}, and SnF \cite{2022SnF}.

%--------------------------------------------------------------------------------------------------------
%%%%% 现有图处理在硬件层次的挑战:computing storage communication
%--------------------------------------------------------------------------------------------------------
\subsection{Challenges in Hardware Level}

%如上所示，图处理算法在硬件上的执行正在面临许多挑战。一般情况下，在硬件层面，问题主要来自3个方面：计算（computing），存储（storage）和通信（communication）。接下来我们关注关键问题的优化目标，从硬件角度分析这些挑战。图global-taxonomy(a)说明了一般的硬件层次：计算方面的挑战存在于计算单元(a)和多节点工作负载(e)，存储方面的挑战存在于片上和片外存储（bcd），通信方面的挑战存出现在多节点系统（fg）
As mentioned above, the execution of graph processing algorithms on hardware are facing many challenges. Generally, according to the hardware hierearchy, the problems mainly come from three aspects: \textbf{computing}, \textbf{storage}, and \textbf{communication}. Then we focus on the optimization targets of key problems and analyze these challenges from the perspective of hardware. Figure \ref{fig:global-taxonomy} (a) shows a general hardware hierarchy: Challenges for computing resides in computing unit on a single machine(a) and multi-node workloads(e), challenges for storage resides in on-chip and off-chip storage (bcd), challenges for communication arises in multi-core systems (fg). 

%--------- 计算方面的的挑战
\textbf{Challenges for Computing}

%随着数据规模的爆发式增长，大规模图应用倾向于使用多节点系统进行并行计算。 如果不同节点的数据量不统一，节点之间的工作量就会不平衡，这意味着工作量小的核心必须等待工作量大的核心，造成资源浪费。 然而，图结构的不规则性使得图数据难以均匀划分。 此外，图算法大多是计算密集型的，因此大规模的计算数据会消耗大量的计算资源。 同时，计算复杂的图往往会导致大量的冗余操作，使得计算单元的执行效率低下。
With the explosive growth of data scale, large-scale graph applications tend to use multi-node systems for parallel computing. If the data amount in different nodes is not uniform, the workload between nodes will be unbalanced, which means cores with small workloads had to wait for the cores with heavy workloads, resulting in a waste of resources. However, the irregularity of the graph structure makes it difficult to evenly divide the graph data. In addition, graph algorithms are mostly computationally intensive, so large-scale computing data consumes a lot of computing resources. At the same time, computing complex graphs often leads to a large number of redundant operations, making the low execution efficiency of computing units.

%--------- 存储方面的挑战
\textbf{Challenges for Storage}

%存储面临两个主要挑战：1）图结构的不规则性导致缓存利用率低，导致缓存频繁更换，造成大量低效和重复的数据传输。 2）片上内存空间不足，导致很多大型应用无法部署在资源受限的设备上，导致可扩展性差。 即使大规模图通过数据分块运行在小内存设备上，片内缓存不足也会导致片内片外数据交换频繁。 由于图形数据不规则，片外带宽利用率极低。 片外内存访问的速度远低于片内，因此频繁的片外内存访问极大地限制了算法的执行速度，甚至成为整体加速的瓶颈。
There are two main challenges for storage: 1) The irregularity of the graph structure leads to low cache utilization, resulting in frequent cache replacements which causes a large amount of inefficient and repeated data transfer. 2) Insufficient on-chip memory space prevents many large-scale applications from being deployed on resource-constrained devices, resulting in poor scalability. Even if large-scale graphs run on small-memory devices through data blocking, insufficient on-chip caches will lead to frequent on-chip and off-chip data exchanges. Due to irregular graph data, off-chip bandwidth utilization is extremely low. The speed of off-chip memory access is much lower than that of on-chip ones, so frequent off-chip memory access greatly limits the execution speed of the algorithm, and even becomes the bottleneck of the overall acceleration.

%通信方面的挑战
\textbf{Challenges for Communication}

%通信方面的挑战为分布式系统中高昂的数据同步开销。大规模的图数据处理很难在单节点系统上执行，因此多节点分布式图处理的应用愈发广泛。
%由于算法执行时遍历的顶点可能分布在不同节点，导致节点间频繁的数据交换。由于图的不规则性，遍历也是不规则的，因此通信带宽利用率低。
%某些工作在各节点进行独立的mini-batch训练以避免节点间遍历，然而每次迭代间的参数同步仍然是一项耗时的工作。
The challenge for communication is the high data synchronization overhead in distribution systems. Large-scale graph data processing can hardly execute on a single-node system, so multi-node distributed graph processing are becoming more and more widely used. Since vertices traversed in execution may be distributed in different nodes, frequent inter-nodes data exchange is required. Due to the irregularity of the graph structure, the traversal is also irregular, resulting in a waste of communication bandwidth. Some works perform independent mini-batch training on each node to avoid inter-node traversal, however it is still a time-consuming task of parameters synchronization between iterations.

\begin{figure}[ht]
    \centering
    \vspace{-0.2cm}  %调整图片与上文的垂直距离
    \setlength{\abovecaptionskip}{0cm}     %调整图片标题与图距离
    \setlength{\belowcaptionskip}{0cm}   %调整图片标题与下文距离
    \includegraphics[width=\textwidth]{fig-background/global-taxonomy.eps}
    \caption{Global Taxonomy: (a) Hardware Hierarchy: a-d represent the organizational structure within a single processor, e-g represent the organizational structure in a multi-core system. (b) Taxonomy: Graph Preprocessing Methods are classified in three categories based on the optimization targets}
    \label{fig:global-taxonomy}
\end{figure}

%------------------------------------------------------------------
%%%%% Taxonomy
%------------------------------------------------------------------
\subsection{Taxonomy of Graph Preprocessing Methods }
\label{taxonomy}

%我们在本节中介绍我们的分类法。 为了系统地介绍图预处理方法对硬件层面的影响，我们将图预处理方法分为 3 类：高效计算（efficient computing）、高效存储（efficient storage）和高效通信（efficient communication）的预处理方法。 我们的分类法基于从上述挑战中总结的优化目标。
Our taxonomy is shown in Figure \ref{fig:global-taxonomy}. To systematically introduce the impact of graph preprocessing methods on the hardware level, we classify graph preprocessing methods into 3 categories: Preprocessing methods for \textbf{efficient computing}, \textbf{efficient storage}, and \textbf{efficient communication}. Our taxonomy is based on the optimization targets summarized from the challenges above.

%可以从两个方面提高计算效率：负载均衡（load balance），减少计算量（reduce computation）。
%实现负载均衡的关键是形成合理的数据分布，可以通过partition来实现。
%为了减少计算，有许多方法可用。 一方面，我们可以通过采样、稀疏化、压缩等方式减少数据量；另一方面，我们可以通过合并中间结果或降低数据精度来简化计算过程。
\textbf{Computing efficiency} can be raised from two aspects: \textbf{load balance} and \textbf{reduce computation}. The key to achieve load balance between multi-nodes is to form a reasonable distribution of data, which can be achieved by graph partition. To reduce computing, numerous methods are available. On the one hand, we can reduce the amount of data by sampling, sparsification, and quantization. On the other hand, we can simplify the computing process by merging intermediate results (reconstruction) or reduce data precision (quantization).

%可以从2个方面优化存储效率：reduce capacity requirement、reduce data movement.
%容量需求特指所需的片上存储空间。采样、稀疏化和量化可以有效降低数据量，缓解存储压力。
%数据移动是指不同存储层次结构之间的数据流动，其效率可以通过提高片上缓存利用率和片外带宽利用率来优化。 图reorder、图reconstruction和数据blocking 通常用于优化存储访问效率。
\textbf{Storage efficiency} can be optimized from two aspects: \textbf{reduce capacity requirement} and \textbf{reduce data movement}, and reduce access latency. Capcity requirement refers to the required on-chip memory space. Sampling, sparsification, and quantization can effectively reduce data amount and relieve storage pressure. Data movement refers to the data flow between different storage hierarchy, whose efficiency can be optimized by improve on-chip cache utilization and off-chip bandwidth utilization. Graph reorder, graph reconstruction and data blocking are commonly used to optimize storage access efficiency.

%可以从2个方面提高通信：reduce communication frequency、reduce communication latency。
%通信是指分布式系统中节点之间的数据传递，其效率低下的原因在于节点之间频繁且不规律的数据交换。
%提高数据局部性可以大大降低节点间通信频率，这可以通过分割（partition）实现。
%数据的并行重新排序有助于提高通信带宽利用率，进而减少端到端时间，执行高效的数据传递以提高通信效率。
\textbf{Communication efficiency} can be improved from two aspects: \textbf{reduce communication frequency} and \textbf{reduce communication latency}. Communication refers to the data passing between nodes in distributed systems, whose inefficiency comes from frequent and irregular data exchange between nodes. Improving data locality can greatly reduce the communication frequency between nodes, which can be achieved by parititon. Parallel reorder of data helps to improve communication bandwidth utilization, thereby reducing end-to-end time, performing efficient passing of data to improve communication efficiency.

%对于每个类别，我们将在Section（Category）中进行详细说明，并从多个方面比较预处理方法。
We will elaborate each category in detail in Section \ref{category} and compare preprocessing methods in multiple aspects.













==> old/category-hardware-old.tex <==
%在上一节中，我们分析了在硬件层面遇到的挑战，将三个优化目标作为我们的分类法，即计算、存储和通信。在本节，我们将按分类介绍预处理方法。对于每个类别，我们详细阐可行的优化策略，并列举可用的预处理方法。
In the previous section, we analyze challenges encountered in hardware level, taking three optimization targets as our taxonomy which are computing, storage, and communication. In this section, we introduce preprocessing methods by category. For each category, we elaborate the corresponding optimization strategies and example available preprocessing methods. We list and describe various works with these preprocessing methods, and then compare them in multiple dimensions.

%Since most preprocessing methods are only applicable to traditional graph processing algorithms or graph neural network algorithms, we will introduce the preprocessing methods of the two respectively, and conduct a comparative analysis.

%------------------------------------------------------------------
%%%%% Efficient Computing：
%     1. load balance 
%     2. reduce computation
%------------------------------------------------------------------
\subsection{Preprocessing Methods for Efficient Computing}

%如上x节所述，我们可以从两个方面提高计算效率：一是提高计算单元的整体执行效率，这可以通过load balance来实现； 二是减少执行所需的数据量，即通过reduce computation来削减算法运行开销。
%下面我们将介绍通过预处理提高计算效率的典型工作。
As illustrate in section \ref{taxonomy} above, we can improve computing efficiency from two aspects: one is to improve the overall execution efficiency of computing unit, which can be achieved through \textit{load balance}; two is to reduce the amount of data required for execution, which is to cut algorithm running overhead through \textit{reduce computation}. Next, we will introduce some typical works which improve computing efficiency through preprocessing.

\begin{table*}[h]
\vspace{-0.15cm}  %调整表格与上文距离
\caption{Preprocessing Methods for Efficient Computing}
\vspace{-0.3cm}  %调整表格标题距离
\label{table:Efficient-computing}
\renewcommand{\arraystretch}{1.2}%调行距
\setlength\tabcolsep{10pt}%调列距
\begin{tabular}{cccc}
\toprule
Target     & Method   & Algorithm     & Paper     \\
\midrule
\multirow{2}{*}{Load Balance}        
& \multirow{2}{*}{Partition} & Traditional & METIS\cite{1998METIS} \\
&                            & GNN         & DistDGL\cite{2020DistDGL}, PaGraph\cite{2020PaGraph} \\
\midrule
\multirow{4}{*}{Reduce Computation}  
& Sparsification & GNN & DropEdge\cite{2020DropEdge}, GLT\cite{2021GLT} \\
\cline{2-4}
& Reconstruction & GNN & GraphAct\cite{2020GraphACT}, GCNInference\cite{2020GcnInference}  \\
\cline{2-4}
& Sampling       & GNN & GraphSage\cite{2017graphsage}, FastGCN\cite{2018FastGCN}          \\
\cline{2-4}
& Quantization   & GNN & Bi-GCN\cite{2021Bi-GCN}, DegreeQuant\cite{2020DegreeQuant}        \\
\bottomrule
\end{tabular}
\vspace{-0.15cm}  %调整表格与下文距离
\end{table*}

%-------------------- efficient computing: load balance --------------------%
\noindent{\textit{A. Load Balance}}

%现实生活中的图具有大规模的数据，因此很难在单核上运行图处理算法。由于图结构不规则，不同顶点的程度差异很大，很难将顶点均匀分布到不同的计算核上，导致不同计算核的工作量差异很大。因此工作量小的核需要等待工作量大的计算核心，造成局部热点。为了避免这种计算资源的浪费，许多工作使用partition方法进行负载平衡，这被广泛用于加速传统的图算法和图神经网络算法。
Real-life graphs have large scale data, so it is difficult to run graph processing algorithms on a single core. Since different vertices vary dramatically in degree with the irregularity graph structure, it is difficult to evenly distribute vertices to different computing cores, which leads to great workload differences in different computing cores. Therefore, cores with lighter workloads need to wait for cores with heavier workload, causing local hot spots. To avoid this waste of computing resources, many works use \textbf{partition} methods for load balance, which is widely used to accelerate traditional graph algorithms and graph neural network algorithms.

\textbf{a) Partition for load balance}

%为了将一个大图数据均匀地分配给k个计算核，一个经典的方法是构造一个平衡的k-way edge-cut，其中顶点被平均分成k个互斥的部分（称为分区P），切割的边数量最少。 顶点代表计算任务，边代表数据交换。 由于每个核包含大约相同数量的顶点，因此工作负载是平衡的，同时，最少数量的跨越core的边减少了数据交换. k-way划分的过程如下
To evenly allocate a large graph data to k computing cores, a classic way is to construct a balanced k-way edge-cut, in which vertices are evenly divided into k mutually-exclusive parts (called partition \textit{P}) with a minimal number of cutting edges. The vertices represent computing tasks, and the edges represent data exchange. The workload is balanced since each core contains about the same number of vertices,  meanwhile, the data exchange is decreased with a minimal number of edges spanning cores. The process of k-way partition is as follows:

\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:partition}
Partition(\textit{V})= \{{\bigcup}_{i} \textit{V}_\textit{i} \vert i=1,\cdots,\textit{k}; \forall i \neq j, \textit{V}_\textit{i} \cap \textit{V}_\textit{j} = \emptyset, \}% \textit{V}_1 \cup \textit{V}_2 \cdots \cup \textit{V}_\textit{k} \{\textit{V}_\textit{i} \cap \textit{V}_\textit{j} = \emptyset, \forall i \neq j\}
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}

%1)METIS[]是一种multilevel graph partition方法，如图x(a）整体过程包含3个步骤:coarsening，partitioning，uncoarsening。在coarsening阶段，Gi的顶点集合并形成下一级图Gi+1的新顶点(如图x(b)所示)，输入图G0经过中间较小的图G1,G2,...Gm被逐渐转化为很coarse的图Gm。在划分阶段，对小图Gm进行k路划分，Pm是Gm的局部最小划分(local minimum partition）。在uncoarsening阶段，粗粒度图Gm的划分Pm将通过一系列划分Pm-1,Pm-2,...,P0逐渐被映射回原始图。Pi到Pi-1的过程中，先完成顶点映射，然后执行启发式的refinement算法对边界点进行优化，以减少edge-cut。
1) METIS\cite{1998METIS} is a multilevel graph partition method, as shown in Figure \ref{fig:METIS} (a). The overall process includes three steps: coarsening, partitioning, and uncoarsening. In the coarsening phase, vertices sets of $\textit{G}_{i}$ are combined to form new vertices of next level graph $\textit{G}_{i+1}$ (as shown in Figure \ref{fig:METIS} (b)), and the input graph $\textit{G}_{0}$ is gradually transformed into a very coarse graph $\textit{G}_{m}$ by going through intermediate smaller graphs $\textit{G}_{1}$, $\textit{G}_{2}$, ..., $\textit{G}_{m}$. In the parititioning phase, a k-way partition of the coarse graph $\textit{G}_{m}$ is carried out, and $\textit{P}_{m}$ is the local minimum partition of $\textit{G}_{m}$. In the uncoarsening phase, the partition $\textit{P}_{m}$ of $\textit{G}_{m}$ is gradually projected back to the original graph $\textit{G}_{0}$ by going through a sequence of partitions $\textit{P}_{m-1}$, $\textit{P}_{m-2}$, ..., $\textit{P}_{0}$. In process from $\textit{P}_{i}$ to $\textit{P}_{i-1}$, the vertex mapping is completed first, and then a heuristic refinement algorithms is performed to optimize the boundary vertices partition to reduce edge-cut. 

%------- 图片 METIS
\begin{figure}[ht]
    \centering
    \vspace{-0.2cm}  %调整图片与上文的垂直距离
    \setlength{\abovecaptionskip}{0.1cm}     %调整图片标题与图距离
    \setlength{\belowcaptionskip}{-0.2cm}   %调整图片标题与下文距离
    \includegraphics[width=\textwidth]{fig-category/METIS.eps}
    \caption{The partition process of METIS: (a) The phases of the multilevel graph partition; (b) Coarsening phase}
    \label{fig:METIS}
\end{figure}

%METIS 是一种典型的边切分区方法，在许多工作中被广泛使用。 由于其旨在获得顶点负载平衡，因此更适用于划分稀疏图。 如果顶点度数高，大量的边切割会带来沉重的通信负担。 由于METIS需要遍历整个图，对于大规模图来说需要很高的时间和内存开销，所以METIS通常被用作离线预处理。
METIS is a typical edge-cut partition method which is commonly used in many works. For it aims to gain a vertices load balance, it is more applicable to divide sparse graphs. If vertices has high degrees, the large number of edge-cut will bring heavy communication burden. Since METIS needs to traverse the whole graph, it takes a high time and memory overhead for large scale graphs, so METIS is usually used as an offline preprocessing.

%2)DistDGL[]是一个分布式GNN训练框架，使用同步随机梯度下降（SGD）进行训练。 这种训练方式需要生成一个平衡的mini-batch进行训练，即每个mini-batch包含大致相同数量的顶点和边，并从网络中读取大致相同数量的数据。 DistDGL 首先使用 METIS 进行图分区，然后在每个分区中采样多个小批量进行训练。 为了使训练者拥有相同数量的训练样本，DistDGL 采用了two-level策略，将数据集平均分配给所有训练者。 它首先完成顶点划分（如图x），这些顶点称为核心顶点，然后将核心顶点的源顶点复制到每个部分，称为HALO顶点。 在完成图结构划分后，DistDGL将核心顶点和边的特征分配给每个部分，使得顶点和边的特征不重复。这样，DistDGL 改进了原有的 METIS，解决了训练过程中图划分的边平衡问题。
2) DistDGL\cite{2020DistDGL} is a distributed GNN training framework which uses synchronized stochastic gradient descent (SGD) for training. This training way needs to generate a balanced mini-batch for training, that is, each mini-batch contains roughly the same number of vertices and edges, and reads roughly the same amount of data from the network. DistDGL first uses METIS for graph partitioning, and second samples multiple mini-batches in each partition for training. In order to make trainers have a same number of training samples, DistDGL uses a two-level strategy to evenly distribute the data set to all trainers. It first completes vertices division (as shown in Figure \ref{fig:DistDGL}), these vertices are called core vertices, and then duplicate the source vertices of core ones to each part, called HALO vertices. After completing the graph structure partition, DistDGL assigns features of the core vertices and edges to each part, so that the features of vertices and edges are not repeated. In this way, DistDGL improves original METIS, solving the edge balance problem of graph partitioning in training process.

%------- 图片 DistDGL
\begin{figure}[ht]
    \centering
    \vspace{-0.2cm}  %调整图片与上文的垂直距离
    \setlength{\abovecaptionskip}{0.1cm}     %调整图片标题与图距离
    \setlength{\belowcaptionskip}{-0.2cm}   %调整图片标题与下文距离
    \includegraphics[width=0.8\textwidth]{fig-category/DistDGL.eps}
    \caption{Graph parititioning with METIS in DistDGL: (a) Assign vertices to graph parititions; (b) Generate graph partitions with HALO vertices (the vertices with different colors in the parition is HALO vertices)}
    \label{fig:DistDGL}
\end{figure}

%3) 3)PaGraph[] 是一个支持在具有多 GPU 的单服务器上进行 GNN 训练的系统。与 DistDGL[] 类似，每个 GPU 分配一个子图进行独立训练，然后每次迭代同步更新训练参数。 为了平衡训练工作量，需要将图平均划分为 K 个分区。 在划分过程中，它扫描整个训练顶点集，并将扫描的顶点迭代地分配到一个分区中。 每次迭代都会计算出每个顶点的得分，如式xx所示： TVi表示分配给分区i的顶点集； PVi 表示分区 i 中的顶点总数，vt 最有可能分配给 PV 最小的分区。 TVavg 是每个分区中训练顶点的预期数量，设置为|TV|/K 用于负载平衡。
3) PaGraph\cite{2020PaGraph} is a system that support GNN training on a single server with multi-GPU. Similar to DistDGL\cite{2020DistDGL}, each GPU is allocated an subgraph for independent training, then updates the training parameters synchronously per iteration. To balance the training workload, the graph is evenly divided into \textit{K} partitions. In partition process, it scans the whole training vertex set, and iteratively allocates the scanned vertices to one partition. Each iteration will calculate the score of each vertex which is shown in Equation \ref{equation:score}: $\textit{TV}_\textit{i}$ represents the vertex set allocated to partition \textit{i}, $\textit{PV}_\textit{i}$ represents the total number of vertices in partition \textit{i}, and $\textit{v}_\textit{t}$ is most likely allocated to the partition with the smallest \textit{PV}. $\textit{TV}_\textit{avg}$ is the expected number of training vertices in each partition which is set as $\frac{\vert\textit{TV}\vert}{\textit{K}}$ for load balance.

\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:score}
\textit{score}_{\textit{v}_\textit{t}}^{(\textit{t})} = \vert\textit{TV}_\textit{i} \cap \textit{IN}(\textit{V}_\textit{t})\vert \cdot \cfrac{\textit{TV}_\textit{avg}-\vert\textit{TV}_\textit{i}\vert}{\vert\textit{PV}_\textit{i}\vert}
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}

%算法 1 展示了整个分区过程，它基于线性确定性贪婪算法 (LDG)。 在每次迭代中，它计算每个顶点的得分并从中导出目标分区索引ind（line4），然后将顶点vt及其N-hop邻居分配给Gind（line5）。 由于这个图分区是离线预处理，只在训练前执行一次，所以额外的时间和资源消耗是可以接受的。
Algorithm \ref{alg:PaGraph} presents the whole partition process, it is based on Linear Deterministic Greedy (LDG). In each iteration, it calculates the score of each vertex and derives the target partition index \textit{ind} from which (line4), and then allocates the vertex $\textit{v}_\textit{t}$ and their \textit{N}-hop neighbors to $\textit{G}_\textit{ind}$ (line5). Since this graph partition is offline preprocessing which only executes once before training, so the extra time and resource consumption is acceptable. 

\begin{algorithm}[H]
%\SetAlgoNoLine  %去掉之前的竖线
\caption{Computing-balanced graph partition using score vector in PaGraph}
\label{alg:PaGraph}
\KwIn{Graph \textit{G}, Vertex set \textit{TV}, Number of hops \textit{N}, Partition number \textit{K}}
\KwOut{Graph partition $\textit{P}_1, \textit{P}_2, ...,\textit{P}_\textit{K}$}
\lFor{$\textit{i} \leftarrow$ 1 to $\textit{K}$}{$\textit{P}_\textit{i} \leftarrow \varnothing$; // Initialization}
\ForEach{$\textit{v}_\textit{t} \in \textit{TV}$}
{
    $\textit{IN}(\textit{v}_\textit{t}) \leftarrow \textit{IN-NEIGHBOR}(\textit{v}_\textit{t}, \textit{G}, \textit{N})$; \\
    
    $\textit{ind} \leftarrow arg max_{\textit{t} \in [1,\textit{K}]}\{\textit{score}_{\textit{v}_\textit{t}}^{(\textit{i})}\}$, 
   $\textit{score}_{\textit{v}_\textit{t}} \leftarrow SCORE(\textit{v}_\textit{t}, \textit{IN}(\textit{v}_\textit{t}))$; \\
    $\textit{G}_\textit{ind} \leftarrow \textit{G}_\textit{ind} \cup \{\textit{v}_\textit{t}\} \cup \{\textit{IN}(\textit{v}_\textit{t})\}$;
}
\Return $\{\textit{P}_1, \textit{P}_2, ...,\textit{P}_\textit{K}\}$
\end{algorithm}

\textbf{b) Comparisons of methods for load balance} 
\todo{time complexity O(n)}

%-------------------- efficient computing: reduce computation --------------------%
\noindent{\textit{B. Reduce Computation}}

%为了将 GNN 用于更高级的研究应用，GNN 模型变得越来越复杂。 随着图规模的爆炸式增长，GNN 算法执行中的计算负担变得更加沉重。 但是，设备的计算资源是有限的，很多任务对时间要求严格，海量计算带来的时间和资源消耗往往难以承受。 许多预处理工作通过减少计算来实现 GNN 的加速，这取决于两个事实：1）图聚合阶段收集了大量冗余的顶点和边，可以在不影响最终执行结果的情况下将其移除以减少冗余计算。 稀疏化和重建是去除冗余数据的常用方法。 2）由于神经网络变换中大量的正则计算是在组合阶段进行的，因此可以将NN中常用的采样和压缩方法扩展到GNN中进行加速，从而减少计算开销。
To use GNNs for more advanced research applications, the GNNs models are becoming much more complicated. With the explosive increase of graph scale, the computing burden in GNNs algorithm execution becomes much more heavier. However, the computing resources of the device are limited, and many tasks have strict time requirements so the time and resource consumption caused by massive computing often become unbearable. Many preprocessing works achieve an acceleration of GNNs by reducing computing, which depends on two facts: 1) The graph aggregation stage collects a large number of redundant vertices and edges, which could be removed to reduce redundant computation without affecting the final execution results. Sparsification and reconstruction are common methods for removing redundant data. 2) Since a large amount of the regular computation in the neural network transformation performed in the combination stage, sample and compression methods commonly used in NNs can be extended to GNNs for acceleration, thereby reducing computing overhead.

\textbf{a) Sparsification for reducing computation}

%深度图神经网络面临过度平滑和过度拟合的问题。 图稀疏化可以通过去除边来增加随机性，促进模型收敛。 在计算过程中，稀疏化方法通过建立特定的优化目标，去除与任务无关的边，从而减少冗余计算，加速算法执行。
Deep graph neural networks are faced with over-smoothing and over-fitting problems. Graph sparsification can increase randomness with removing edges, promoting the model convergence. In the computing process, sparsification method removes edges which are task-irrelative by establishing a specific optimization goal, thereby reducing redundant computation to accelerate algorithms execution.

1) DropEdge\cite{2020DropEdge} proposes to randomly remove edges per training epoch, which is implemented by randomly forcing the $\textit{V}_\textit{p}$ non-zero elements in adjacency matrix \textit{A} to be 0, where \textit{V} is the total number of edges, and \textit{p} is the drop rate. In aggregation stage, DropEdge aggregates completely random subsets, which does not change the aggregation expectation, so DropEdge is an unbiased data augmentation technique for GNN training. Different from an global optimization strategy, dropping edges strategy is heuristic in DropEdge, taking both speed and randomness into consideration. More improtant, DropEdge is a generally skill that can be equipped with various models (such as GCN\cite{2017GCN} and GraphSage\cite{2017graphsage}), and it improve the performance on both shallow and deep GCNs.

2) GLT\cite{2021GLT} first extended the lottery ticket hypothesis (LTH) \cite{2018Lottery} to GNNs, and proposed graph lottery tickets (GLT) which is defined as a pair of sub-datasets (core sub-dataset) and sparse sub-network (sparse sub-network). This paper proposes a unified GNN sparsification framework (UGS), which is an end-to-end framework to simultaneously sparse graph adjacency matrix (A) and model weights (W). UGS is applied to iteratively identify GLT from the input graph and the original GNN model. Similar to DNNs, GLTs can be trained from initialization, then matching training performance,full graphs and models. Using GLT can greatly reduce the sparse matrix multiplication (MAC) operations to accelerate the training and inference of GNN. For node classification, GLT saves 20\%~98\% MACs on small graphs and  25\%~85\% MACs on large ones without accuracy-loss.


\textbf{b) Reconstruction for reducing computation}

%由于许多高度顶点共享许多邻居，这些公共顶点将在聚合阶段重复聚合，导致冗余计算。 重构的核心思想是合并共享的邻居，这样可以在不丢失信息的情况下消除冗余计算，提高计算效率。
Since many high-degree vertices share many neighbors, these common vertices would be repeatedly aggregated during the aggregation phase, resulting in redundant computation. The core idea of reconstruction is to merge shared neighbors, so that redundant computation can be eliminated without loss of information, and computing efficiency can be improved.

%------- 图片 graphact
\begin{figure}[ht]
    \centering
    \vspace{-0.2cm}  %调整图片与上文的垂直距离
    \setlength{\abovecaptionskip}{0.1cm}     %调整图片标题与图距离
    \setlength{\belowcaptionskip}{-0.2cm}   %调整图片标题与下文距离
    \includegraphics[width=0.6\textwidth]{fig-category/GraphAct.eps}
    \caption{Reducing redundancy in feature propagation of GraphAct\cite{2020GraphACT}}
    \label{fig:GraphAct}
\end{figure}

%1）GraphACT[]通过预处理提前完成输入图中高复用部分的计算。 如图x所示，预处理阶段识别公共邻居对（图x(b)0和2、1和3），计算邻居对的特征并构造新的子图（图x(c)），其中顶点 0和2，顶点1和3造成重复聚集。 顶点0和2合并为顶点u，顶点1和3合并为顶点v。GraphACT中使用的重构方法是轻量级的，可以在线运行，减少了高达60%的冗余归约操作，从而有效减少了计算。
1) GraphACT\cite{2020GraphACT} completes the computing of the high reuse part in the input graph in advance through preprocessing. As shown in Figure x, the preprocessing stage identifies the common pairs of neighbors (Figure \ref{fig:GraphAct} (b) 0 and 2, 1 and 3), computes features of neighbor pairs and constructs a new subgraph (Figure \ref{fig:GraphAct} (c)), where vertices 0 and 2,  vertices 1 and 3 cause repeated aggregation. Vertices 0 and 2 are merged into vertex \textit{u}, and vertices 1 and 3 are merged into vertex \textit{v}. The reconstruction method used in GraphACT is lightweight and can run online, reducing redundant reduction operations by up to 60\%, thereby effectively reducing the amount of computation.

2) GCNInference\cite{2020GcnInference} adopts a reconstruction method similar to that in GraphACT\cite{2020GraphACT}, which eliminates the redundant edge computing of high degree vertices and improves the computing efficiency. The difference is that GraphACT is used to accelerate GNN training, while the GCNInference is used to accelerate GCN inference. The inference process contains more redundancy compared with the training process with mini-batch, hence graph reconstruction strategy provides more obvious optimization in the inference process. In addition, the graph reconstruction method is also applied in I-GCN\cite{2021I-gcn}, which greatly reduces redundant computation during inference.

\textbf{c) Sampling for reducing computation}

%图的全批训练需要全梯度下降法。 对于复杂的图模型，全梯度法需要在每次更新时计算所有顶点的嵌入。 由于每个epoch只更新一次参数，损失函数收敛很慢，计算效率很低。 因此，研究人员将 mini-batch 策略引入到 GNN 算法中以加速收敛，这被称为图采样。
The full-batch training of the graph requires a full gradient descent method. For complex graph models, the full gradient method needs to compute the embedding of all vertices each update. Since it only updates the parameters once per epoch, the loss function converges very slowly, resulting poor computing efficiency. Therefore, researchers introduce the mini-batch strategy into GNN algorithms to speed up the convergence, which is called graph sampling.

%1)GraphSage[] 首先将mini-batch引入GCN训练，提出了mini-batch SGD。GraphSage使用了一种node-wise的采样方法。如图x所示，GraphSage为每个顶点随机抽取固定的邻居，每次更新只基于一个mini-batch的梯度，每个epoch更新多次，加快了收敛速度，减少了计算开销。和full-batch计算相比，虽然在采样时损失了一些信息，但仍然取得了较好的训练效果。然而，node-wise采样仍存在两个主要问题：1）node-wise方法的邻居成指数增长,随着层数的增加,庞大的顶点数带来沉重的计算开销；2）由于图的幂律性，顶点的度往往不固定，当每个顶点的固定采样数较大时，难免出现大量的重复采样，影响计算效率。 
1) GraphSage\cite{2017graphsage} first introduced mini-batch into GCN training, using stochastic gradient descent (SGD) training instead of full gradient descent training. GraphSage uses a node-wise sampling method, as shown in Figure \ref{fig:sample1}, GraphSage randomly selects fixed neighbors for each vertex. Since each update is only based on the gradient of a mini-batch, each epoch updates multiple times, which speeds up the convergence and reduces computing overhead. Though some information is lost during sampling, it achieves better accuracy compared with full-batch training. However, there are still two main problems in node-wise sampling: 1) The neighbors of the node-wise method grow exponentially, and the huge number of vertices brings heavy computing overhead with layer increasing; 2) Since degree of vertices vary greatly in pow law graph, it is inevitable to select a large number of repeated samples when each vertex samples large number of fixed neighbours. Therefore, a large number of randomly sample may cause redundant computation, resulting lower training efficiency.

%------- 图片 node-wise and layer-wise sample method
\begin{figure}[ht]
    \centering
    \vspace{-0.2cm}  %调整图片与上文的垂直距离
    \setlength{\abovecaptionskip}{0.1cm}     %调整图片标题与图距离
    \setlength{\belowcaptionskip}{-0.2cm}   %调整图片标题与下文距离
    \includegraphics[width=1\textwidth]{fig-category/sample1.eps}
    \caption{Sampling process of node-wise sampling method and layer-wise sampling method.}
    \label{fig:sample1}
\end{figure}

%2)FastGCN[]提出了layer-wise sampling方法，即按照预设的概率分布在每一层独立采样固定数量的顶点，如图x所示。 与邻居数量呈指数增长的逐节点采样不同，逐层采样在每一层采样固定数量的顶点，可以有效地限制邻居的爆炸式增长。 Layer-wise用蒙特卡洛算法估计顶点嵌入，通过上层父顶点的关系对下一层进行采样，大大减少了每一层的重复采样。 但是，由于每一层的采样都是独立的，随着层数的增加，采样的子图变得越来越稀疏，导致最终的计算embedding方差较大。 虽然与逐节点采样相比，逐层采样有效地减少了冗余计算，但它不能采样太多层以保持训练精度。
2) FastGCN\cite{2018FastGCN} proposes a layer-wise sampling method, which is independently samples a fixed number of vertices in each layer according to a preset probability distribution, as shown in Figure \ref{fig:sample1}. Different from node-wise sampling where the number of neighbors increases exponentially, layer-wise sampling samples fixed number of vertices in each layer, which can effectively limit the explosion growth of neighbours. Layer-wise estimates the vertex embedding with Monte Carlo algorithm, and samples the next layer through the relationship of the parent vertex in the upper layer, which greatly reduces the repeated sampling in each layer. However, since the sampling of each layer is independent, the sampled subgraphs become sparser as the number of layers increases, resulting in a large variance in the final computing embedding. Though layer-wise sampling effectively reduces redundant computing compared with node-wise sampling, it could not sample too much layers to maintain training accuracy.

\textbf{d) Quantization for reducing computation}

%GNN 的执行依赖于海量的数据和复杂的模型，这导致了巨大的计算开销。 模型压缩是简化计算过程、减少数据量的有效途径。 典型的压缩方式是量化，已广泛应用于 DNNs[2018CompressionSurvey]。 最近，一些工作将量化方法扩展到 GNN，使用较低精度的模型来实现计算加速，而不会显着降低模型性能。
The execution of GNNs relies on massive data and complex models, which leads to huge computing overhead. Model commpression is an effective way to simplify the computing process and reduce the amount of data. The typical way of compression is quantization, which has been widely used in DNNs\cite{2018NNCompressionSurvey}. Recently, some work has extended the quantization method to GNNs, using lower-precision models to achieve computing acceleration without significantly reducing model performance.

%1）Bi-GCN[]首先将二值化策略引入到图神经网络中，提出了同时对网络参数和输入顶点特征进行二值化的二值图卷积网络。基于向量二值化算法，特征计算公式为：
%β 和 α 分别是 H 和 W 的标量。 由于F(l)和B(l)都是1或-1，所以两个二元向量的内积可以转化为二元运算，即异或和计数运算，特征计算公式转化为
1) Bi-GCN\cite{2021Bi-GCN} first introduces the binarization strategy into the graph neural network, and proposes a binary graph convolutional network which simultaneously binarizes network parameters and input vertex features. Based on the vector binarization algorithm, the feature is calculated by:
\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:binarization1}
\textit{Z}_{\textit{ij}}^{(\textit{l})} = \beta_{\textit{i}}^{(\textit{l})}\alpha_{\textit{i}}^{(\textit{l})}\textit{sign}(\textit{H}_{\textit{i},:}^{(\textit{l})})\cdot\textit{sign}(\textit{W}_{:,\textit{j}}^{(\textit{l})})
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}
$\beta$ and $\alpha$ are the scalar of \textit{H} and \textit{W} respectively. Since $sign(\ast)$ is 1 or -1, the inner product of two binary vectors can be transformed into a binary operation, that is, XNOR and bit counting operations, and the feature calculation formula is transformed into:
\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:binarization2}
\textit{Z}_{\textit{ij}}^{(\textit{l})} = \beta_{\textit{i}}^{(\textit{l})}\alpha_{\textit{i}}^{(\textit{l})}\textit{sign}(\textit{H}_{\textit{i},:}^{(\textit{l})})\otimes\textit{sign}(\textit{W}_{:,\textit{j}}^{(\textit{l})})
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}
Calculated via equation \ref{equation:binarization2}, Bi-GCN changes the original matrix multiplication into a binary operation, achieves a speedup of x53 times of a 2-layer GCN on the Cora dataset. As the depth of GCN increases, the binarized model can get better accuracy.

%2) DegreeQuant[]提出了一种基于度的量化训练方法，使用低精度INT8进行GNN推理。 发现随着入度的增加，聚合的均值和方差会逐渐增大。 为了减轻误差累积，DegreeQuant 使用伯努利分布生成掩码，以全精度计算高入度顶点和低精度计算低入度顶点（图 x）。 实验表明，使用 DegreeQuant 训练的模型的性能接近使用 FP32 训练的模型，并且需要更少的推理时间。
2) DegreeQuant\cite{2020DegreeQuant} proposed a quantized training method based on degree, using low-precision INT8 for GNN inference. It is found that as the in-degree increases, the aggregated mean and variance will gradually increase. To alleviate the error accumulate, DegreeQuant generates a mask using the Bernoulli distribution, calculating high in-degree vertices with full precision and low in-degree ones with low-precision (Figure \ref{fig:DegreeQuant}). Experiments shows that the performance of the model trained with DegreeQuant is close to that trained with FP32, and it require less inference time.

%------- 图片 Degree Quant
\begin{figure}[ht]
    \centering
    \vspace{-0.2cm}  %调整图片与上文的垂直距离
    \setlength{\abovecaptionskip}{0.1cm}     %调整图片标题与图距离
    \setlength{\belowcaptionskip}{-0.2cm}   %调整图片标题与下文距离
    \includegraphics[width=0.7\textwidth]{fig-category/DegreeQuant.eps}
    \caption{Degree-based Quantization method: High in-degree vertices (black) operate at full precision and Low in-degree vertices (grey) operate at reduced precision.\cite{2020DegreeQuant}}
    \label{fig:DegreeQuant}
\end{figure}

\textbf{e) Comparisons of methods for reducing computation}
\todo{time complexity O(n)}

%------------------------------------------------------------------
%%%%% Efficient storage：
%     1. reduce capacity requirement
%     2. reduce data movement
%------------------------------------------------------------------
\subsection{Preprocessing Methods for Efficient Storage}

%如第 x 节所示，存储压力来自片上内存不足和数据访问带宽利用率低。 要实现高效存储，一方面可以通过降低存储需求来缓解片上缓存压力； 另一方面，我们可以减少需要访问的数据量，以减少频繁数据移动的开销。 接下来我们详细介绍提高存储效率的典型的预处理工作。
As illustrated in Section \ref{taxonomy}, the pressure on storage comes from the insufficiency of on-chip memory and low utilization of data access bandwidth. To achieve efficient storage, on the one hand, we can alleviate the on-chip cache pressure by reducing storage requirements; on the other hand, we can reduce the amount of data required access to reduce the overhead of frequent data movement. Next we detail typical preprocessing works to improve storage efficiency.

%-------------------------- Effecient storage 整体表格 --------------------------------%
\begin{table*}[h]
\vspace{-0.15cm}  %调整表格与上文距离
\caption{Preprocessing Methods for Efficient Storage}
\vspace{-0.3cm}  %调整表格标题距离
\label{table:Efficient-storage}
\renewcommand{\arraystretch}{1.2}%调行距
%\setlength\tabcolsep{20pt}%调列距
\begin{tabular}{cccc}
\toprule
Target         & Method    & Algorithm     & Paper \\
\midrule
\multirow{3}{*}{Reduce Capacity Requirement}  
& Quantization    & GNN & SGQuant\cite{2020SGQuant}, EXACT\cite{2021EXACT} \\
\cline{2-4}
& Sampling        & GNN & Cluster-GCN\cite{2019Cluster-GCN} \\
\cline{2-4}
& Sparsification & GNN   & DropEdge\cite{2020DropEdge}, GLT\cite{2021GLT}, AdaptiveGCN\cite{2021Adaptivegcn}   \\
\midrule
\multirow{5}{*}{Reduce Data Movement}  
& \multirow{2}{*}{Reorder}  & Traditional & Gorder\cite{2016Gorder}, ReorderHC\cite{2018ReorderHC}, DBGreorder\cite{2019DBGreorder} \\
&                           & GNN         & Rubik\cite{2021rubik}, GcnInference\cite{2020GcnInference} \\
\cline{2-4}
& \multirow{2}{*}{Blocking} & Traditional &  Graphchi\cite{2012graphchi}, TurboGraph\cite{2013TurboGraph} \\
&                                & GNN        &  HyGCN\cite{2020HyGCN}, AWB-GCN\cite{2020awbgcn}, SnF\cite{2022SnF} \\
\cline{2-4}
& Reconstruction                 & GNN        &  HAG\cite{2020Redundancy-free}, GraphAct\cite{2020GraphACT}, GCNInference\cite{2020GcnInference} \\
\bottomrule
\end{tabular}
\vspace{-0.15cm}  %调整表格与下文距离
\end{table*}

%-------------------- efficient storage: capacity requirement --------------------%
\noindent{\textit{A. reduce capacity requirement}}

%图神经网络往往具有高维特征向量，因此在计算过程中往往需要缓存大量的中间结果，这使得许多大型应用无法部署在存储空间有限的设备上。 片内存储不足导致片内片外数据交换频繁，带来大量额外的内存访问开销。 由于内存访问速度远低于计算单元的执行速度，大量的数据交换甚至可能成为整个运行流水线的瓶颈。 为此，许多工作致力于降低 GNN 的内存消耗，典型的方法包括压缩和采样。
Graph neural networks often have high-dimensional feature vectors, so a large number of intermediate results often need to be cached during the computing process, which prevents many large-scale applications from being deployed on devices with limited storage space. Insufficient on-chip storage causes frequent on-chip and off-chip data exchange, which brings a lot of additional memory access overhead. Since the memory access speed is much lower than the computing units execution speed, a large amount of data exchange may even become the bottleneck of the overall operation pipeline. To this end, many works have been devoted to reducing the memory consumption of GNN, and typical methods include compression and sampling.

\textbf{a) Quantization for reducing capacity requirement}

%GNN的数据输入包括图拓扑和顶点特征，由于GNN特征维度较大，随着顶点数量的增加，整体数据量会急剧增加。压缩可以有效减少整体数据量，降低所需的缓存空间，量化则是最典型的压缩方式。值得注意的是，量化通过大幅度缩减精度来减少存储需求，但往往会带来精度损失，因此相关工作往往需要在内存节约和精度保证之间寻求平衡。
The data input of GNNs includes graph topology and vertex features. Due to the large dimension of GNN features, the overall data volume will increase sharply as the number of vertices increases. Compression can effectively reduce the overall data volume and reduce the required cache space, and quantization is the most typical compression method. It is worth noting that quantization reduces storage requirements by greatly reducing precision, it often brings accuracy loss, so related work often needs to find a balance between memory saving and accuracy assurement.

%1)SGQuant 提出了一种专门的 GNN 量化方法来压缩顶点特征。 为了减少精度损失，它根据量化参数微调 GNN 模型。 作者提出了一种多粒度量化策略（layer-wise、component-wise 和 topology-aware 3 种粒度），可以自动压缩特征数据并最大限度地减少精度损失。 为了最大限度地减少设计探索的工作量，作者基于 ML 自动位选择 (ABS) 为量化粒度选择最合适的位数。 使用 SGQuant 方法，内存使用量减少了 4.25~31.9 倍，精度损失小于 0.4%。
1) SGQuant\cite{2020SGQuant} proposes a dedicate GNN quantization method to compress vertex features. To reduce accuracy loss, it fine tunes the GNN model according to the quantization parameters. The author proposes a multi-granularities quantization strategy (layer-wise, component-wise and topology-aware 3 granularities), which can automatically compress feature data and minimize accuracy loss. In order to minimize the workload of design exploration, the author selects the most appropriate number of bits for the quantization granularity based on ML automatic bit-selecting (ABS). Using SGQuant method, the memory usage is reduced by a factor of 4.25~31.9 with an accuracy loss of less than 0.4%.

%2)EXACT[]是一个内存高效GNN训练框架。对于大规模图，GNN的递归邻居聚合需要缓存大量的中间顶点嵌入，使用压缩激活可以有效节省内存开销。EXACT结合了量化和随机投影两种方法来压缩激活，在正向传播时只需要缓存压缩后的激活，正向公式如下：
%在反向传播时，顶点嵌入通过反量化(dequantization)和反投影(inverse projection)恢复，公式如下:
%通过量化投影后的特征向量，EXACT可以达到很高的压缩比，大幅度降低存储需求。使用EXACT训练GNN，激活的内存占用减小了多达32倍，而精度下降控制在0.2%~0.5%。
2)EXACT[] is a memory efficient GNN training framework. For large-scale graphs, recursive neighbor aggregation of GNNs needs to cache a large number of intermediate vertex embeddings, and using compressed activations can effectively save memory overhead. EXACT combines quantization and random projection to compress the activation. During forward propagation, only the compressed activation needs to be cached. The forward formula is as follows:
\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:EXACT_1}
\tilde{\textit{\textbf{h}}}_\textit{v}^{(\textit{l})} = Quant(RP(\textit{\textbf{h}}_\textit{v}^{(\textit{l})}))
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}
During backward propagation, the vertex embeddings are restored by dequantization and inverse projection. The backward formula is as follows:
\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:EXACT_2}
\hat{\textit{\textbf{h}}}_\textit{v}^{(\textit{l})} = IRP(Dequant(\tilde{\textit{\textbf{h}}}_\textit{v}^{(\textit{l})}))
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}
By quantizing the projected feature vectors, EXACT achieves a high compression ratio and greatly reduce storage requirements. Using EXACT to train GNNs, the memory usage of activation is reduced by up to 32 times, and the accuracy drop is controlled at 0.2\%~0.5\%.

\textbf{b) Sampling for reducing capacity requirement}

%对于原始的full-batch训练，每个epoch都需要缓存计算出的全部顶点嵌入，导致高额的缓存开销。而基于采样的mini-batch方案在一个iteration中就会完成参数更新，因此只需要缓存当前迭代的mini-batch的顶点嵌入即可，极大的降低了缓存需求。
For the original full-batch training, it needs to cache all the calculated vertex embeddings each epoch, resulting in high cache overhead. The mini-batch method based on sampling will complete parameter update in one iteration, so only the vertex embeddings of the current iteration mini-batch needs to be cached, which greatly reduces the cache requirement.

%------- 图片 ClusterGCN
\begin{figure}[ht]
    \centering
    \vspace{-0.2cm}  %调整图片与上文的垂直距离
    \setlength{\abovecaptionskip}{0.1cm}     %调整图片标题与图距离
    \setlength{\belowcaptionskip}{-0.2cm}   %调整图片标题与下文距离
    \includegraphics[width=0.7\textwidth]{fig-category/ClusterGCN.eps}
    \caption{The neighborhood expansion difference between traditional GCN (a) and Cluster-GCN (b)\cite{2019Cluster-GCN}. The black vertex is the starting vertex for neighborhood expansion.}
    \label{fig:ClusterGCN}
\end{figure}
%1)1）Cluster-GCN[]基于子图进行采样，使用图聚类算法生成batch进行训练，有效降低了存储压力。首先，Cluster-GCN将原始图划分为c个cluster；然后随机抽取q个簇以及它们的簇间连接构建为一个子图，每个子图作为一个batch进行训练。为了降低分割时簇间边的损失，Cluster-GCN使用图聚类算法构造顶点分区，使同一分区中顶点之间的图连接比不同分区中的顶点之间的图连接更多。如图x所示，基于子图的训练避免了子图外的邻域搜索，缓解了node-wise采样带来的邻域扩展问题。由于每个batch只有一个子图被加载到GPU内存中，而非原始图，极大的降低了Cluster-GCN的内存需求。
1) Cluster-GCN\cite{2019Cluster-GCN} samples based on subgraphs, using graph clustering algorithm to generate batches for training, which effectively reduces storage pressure. Cluster-GCN first divides the original graph into \textit{c} clusters, then randomly selects \textit{q} clusters and their inter-cluster connections to construct a subgraph, each of which is trained as a batch. To reduce the loss of inter-cluster edges during edge-cut, Cluster-GCN uses graph clustering algorithm to construct vertex partitions, so that there are much more graph connections within a part than that between different parts. As shown in Figure \ref{fig:ClusterGCN}, subgraph-based training avoids the neighborhood search outside the subgraph and alleviates the neighborhood expansion problem caused by node-wise sampling. Since only one subgraph is loaded into the GPU memory per batch instead of the original graph, the memory requirements of Cluster-GCN are greatly reduced.

\textbf{c) Comparisons of methods for reducing capacity requirement}

\todo{time and memory complexity O(n)}

%------------------------ efficient storage: data movement -----------------------%
\noindent{\textit{B. Reduce data movement}}

%图处理算法的执行依赖于海量数据和复杂模型。 在算法执行过程中，计算单元需要频繁访问数据。 由于图结构的不规则性，数据访问往往是低效和不规则的。 许多工作通过减少这些低效数据访问来实现计算加速，这来自两个事实：1）图数据在内存中的不规则分布导致缓存命中率低，导致频繁更换缓存。 因此，降低缓存未命中率可以减少从主存到缓存的拷贝数。 由于缓存访问是以缓存行的形式进行的，提高数据局部性可以有效降低缓存未命中率。 重新排序和重排方法可以有效地提高数据局部性和带宽利用率。 2）图数据存在大量冗余操作，部分数据重用率高，导致数据重复访问。 重构可以提前合并复用率高的部分，从而减少重复的数据传输。
Graph processing algorithms execution relies on massive amounts of data and complex models. During algorithm execution, computing units require frequent data access. Due to the irregularity of graph structure, the data access tends to be inefficient and irregular. Many works achieve computing acceleration by reducing these inefficient data access, which comes from two facts: 1) The irregular distribution of graph data in memory leads to low cache hit rate, resulting in frequent cache replacement. Therefore, reducing the cache miss rate can reduce the number of copies from main memory to cache. Since cache access is performed in the form of cachelines, improving data locality can effectively reduce the cache miss rate. Reorder and rearrangement methods can effectively improve data locality and bandwidth utilization. 2) There are a large number of redundant operations in graph data, so some data has a high reuse rate, resulting in repeated data access. Reconstruction can merge parts which have high reuse rate in advance, thereby reducing the repeated data transfers.

\textbf{a) Reorder for reducing data movement}

%图数据的不规则性导致大量的不规则存储，造成内存访问时带宽的浪费。 提高缓存效率可以减少额外的数据访问并充分利用带宽。 reorder方法将可能连续频繁访问的部分放在靠近的位置，提高缓存利用率。 对于reorder方法只是调整了输入数据的存储顺序，并没有改变图结构和算法实现。 因此，reorder 可以广泛应用于各种模型，而不会造成精度损失。
The irregularity of graph data leads to a large amount of irregular storage, resulting in a waste of bandwidth during memory access. Improving cache efficiency can reduce additional data access and make full use of bandwidth. The reorder method puts the parts that may be accessed continuous frequently in a close position to improve the cache utilization. For the reorder method only adjusts the storage order of the input data, it does not change the graph structure and algorithm implementation. Therefore, reorder can be widely used in various models with no accuracy loss.

1) RCM

%Gorder 提出了一个基于优先队列的图排序算法（GO-PQ），将经常紧密访问的顶点保持在一个cacheline。由于BFS，DFS，PR，SP等传统算法是基于out-neighbour更新，可以维护顶点的out-neighbour局部性来降低缓存未命中率。定义具有相同的in-neighbour的顶点为同胞（sibling）顶点，使用打分函数S来衡量两个顶点u，v的紧密程度，公式如下：
%其中Ss是u，v的共同邻居数；Sn表示u，v的邻居关系，若存在边（u,v)或(v,u)，Sn=1。为了最大化的挖掘局部性，基于滑动窗口ω来最大化紧密顶点对（closely node pair）的得分总和F。即找到最优排列函数Φ，为每个顶点分配ID。公式如下：
2) Gorder\cite{2016Gorder} proposes a priority queue-based graph reordering algorithm (GO-PQ), which keeps frequently closely accessed vertices in a cacheline. Since traditional algorithms such as BFS, DFS, PR, and SP are based on out-neighbor updates, the out-neighbor locality of vertices can be maintained to reduce the cache miss rate. Vertices with the same in-neighbors are defined as sibling vertices, and the score function S is used to measure the closeness of vertex u and vertex v, the formula is as follows:
\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:Gorder_1}
\textit{S}(\textit{u}, \textit{v}) = \textit{S}_\textit{s}(\textit{u}, \textit{v}) + \textit{S}_\textit{n}(\textit{u}, \textit{v})
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}
Here $\textit{S}_\textit{s}$ is the number of common in-neighbours of \textit{u} and \textit{v}, $\textit{S}_\textit{n}$ represents the neighbour relationship between \textit{u} and \textit{v} which is 1 if edge (\textit{u}, \textit{v}) or (\textit{v}, \textit{u}) exists. To maximumly exploit locality, the sum of locality score \textit{F} of closely vertex pairs is maximized based on a sliding window $\omega$. That is to find the optimal reorder function $\phi$, and assign different IDs to all vertices. The formula of \textit{F} is as follows:
\begin{center}
\vspace{-0.6cm}  %调整公式与上文距离
\begin{equation}
\label{equation:Gorder_2}
\textit{F}(\phi) = \sum_{0< \phi(\textit{v})-\phi(\textit{u})\le \omega} \textit{S}(\textit{u}, \textit{v})
\end{equation}
\vspace{-0.6cm}  %调整公式与下文距离
\end{center}
%图x显示了图排序的最佳排列，窗口大小ω=3。若要访问顶点v1和v9的out-neighbour，排序前需要访问xxxxxxxxxx，排序后v1只需要访问3个cacheline，v9只需要访问2个。
%Gorder 方法实现了对整个输入图的最优重新排序。 在十亿级别的数据集上，Gorder 将每个缓存级别的缓存未命中率降低了 30-50% 以上，并实现了 1.2-1.5 倍的算法加速。 由于Gorder计算复杂，运行时间长，对大规模图有很好的加速效果。 对于小图，重新排序时间太长以至于得不偿失。
Figure \ref{fig:Gorder} shows the optimal permutation for graph ordering with window size $\omega=3$. To access the out-neighbor of $\textit{v}_1$ and $\textit{v}_9$, it needs to visit all cachelines without reordering. After reordering, $\textit{v}_1$ only needs to visit 3 cachelines, and $\textit{v}_9$ only needs to visit 2 cachelines.
The Gorder method realizes the optimal reorder of the entire input graph. In a billion-level dataset, Gorder reduces cache miss by more than 30-50\% for each cache level, and it achieves a 1.2-1.5 times acceleration for alogrithms. Due to the complex computation and long runtime of Gorder, it achieves a good acceleration for large-scale graphs. For small graphs, the reorder time is too long so that the loss outweighs the gain.

%------- 图片 Gorder
\begin{figure}[ht]
    \centering
    \vspace{-0.2cm}  %调整图片与上文的垂直距离
    \setlength{\abovecaptionskip}{0.1cm}     %调整图片标题与图距离
    \setlength{\belowcaptionskip}{-0.2cm}   %调整图片标题与下文距离
    \includegraphics[width=\textwidth]{fig-category/Gorder.eps}
    \caption{An example of optimal graph reorder of Gorder\cite{2016Gorder}: (a) An graph example and its optimal reordering. (b) Original representation and its optimal reordered representation.}
    \label{fig:Gorder}
\end{figure}

2) DBGreorder\cite{2019DBGreorder}

3) H-GCN\cite{2022H-GCN}

\textbf{b) Blocking for reducing data movement}

%------- 图片 Graphchi
\begin{figure}[ht]
    \centering
    \vspace{-0.2cm}  %调整图片与上文的垂直距离
    \setlength{\abovecaptionskip}{0.1cm}     %调整图片标题与图距离
    \setlength{\belowcaptionskip}{-0.2cm}   %调整图片标题与下文距离
    \includegraphics[width=0.8\textwidth]{fig-category/Graphchi.eps}
    \caption{An example of optimal graph slicing of Graphchi\cite{2012graphchi}}
    \label{fig:Graphchi}
\end{figure}

1) GraphChi\cite{2012graphchi}

2) TurboGraph\cite{2013TurboGraph}

3) HyGCN\cite{2020HyGCN}

4) AWB-GCN\cite{2020awbgcn}

5) SnF\cite{2022SnF}

\textbf{c) Reconstruction for reducing data movement}

1) HAG\cite{2020Redundancy-free}

\textbf{d) Comparisons of methods for reducing data movement}

\todo{time and memory complexity O(n)}


%------------------------------------------------------------------
%%%%% Efficient communication：
%     1. reduce communication frequency
%     2. reduce communication latency
%------------------------------------------------------------------
\subsection{Preprocessing Methods for Efficient Communication}

%如上所述，分布式系统中存在数据同步的昂贵开销。 可以从两个方面提高通信效率：一方面，可以提高不同节点之间的独立性，从而降低通信频率。 另一方面，改善数据局部性以提高通信带宽利用率，从而减少同步期间的通信延迟。
As mentioned in above, there is the expensive overhead of data synchronization in distributed systems. Communication efficiency can be improved from two aspects: On the one hand, the independence between different nodes can be improved, thereby reducing communication frequency. On the other hand, data locality is improved to improve communication bandwidth utilization, thereby reducing communication delay during synchronization.

%-------------------------- Effecient communication 整体表格 ----------------------------------------
\begin{table*}[h]
\vspace{-0.15cm}  %调整表格与上文距离
\caption{Preprocessing Methods for Efficient Communication}
\vspace{-0.3cm}  %调整表格标题距离
\label{table:Efficient-communication}
\renewcommand{\arraystretch}{1.2}%调行距
%\setlength\tabcolsep{20pt}%调列距
\begin{tabular}{cccc}
\toprule
Target         & Method    & Algorithm     & Paper \\
\midrule
\multirow{2}{*}{Reduce Communication Frequency}  
& \multirow{2}{*}{Partition}  & Traditional & Pregel\cite{2010Pregel}, LDG\cite{2012LDG}, PowerGraph\cite{2012powergraph}, NE\cite{2017NE} \\
&                             & GNN         & PCGCN\cite{2020PCGCN}, DistGNN\cite{2021DistGNN}, PipeGCN\cite{2022PipeGCN} \\
\midrule
\multirow{2}{*}{Reduce Communication Latency}  
& \multirow{2}{*}{Reorder}  & Traditional & Gorder\cite{2016Gorder}, ReorderHC\cite{2018ReorderHC}, DBGreorder\cite{2019DBGreorder} \\
&                           & GNN         & Rubik\cite{2021rubik}, GcnInference\cite{2020GcnInference} \\
\bottomrule
\end{tabular}
\vspace{-0.15cm}  %调整表格与下文距离
\end{table*}

%------------ efficient communication: reduce communication frequency ------------%
\noindent{\textit{A. reduce communication frequency}}

%大规模图需要分配给多个节点进行计算。 由于图中度数较多的顶点，很多边被分配给不同的节点，导致执行过程中通信频繁，严重影响系统效率。 划分方法可以提高子图在各个节点中的局部性，减少不必要的数据通信。
Large-scale graphs need to be allocated to multiple nodes for computing. Since there are many high-degree vertices in the graph, many edges are allocated to different nodes, which leads to frequent communication during execution which seriously affects system efficiency. The partition method can improve the locality of the subgraph in each node and reduce unnecessary data communication.

\textbf{a) Partition for reducing communication frequency}

1) Fennel \cite{2014Fennel}

2) DistDGL \cite{2020DistDGL}

3) PaGraph \cite{2020PaGraph}

\textbf{b) Comparisons of methods for reducing communication frequency}

%------------- efficient communication: reduce communication latency -------------%
\noindent{\textit{B. Reduce communication latency}}

%分布式系统中一个顶点的邻居可能存在于不同的节点中，图的不规则性导致的频繁缓存未命中会导致并行处理时大量的核间通信，限制了整体的运行效率。 重排序虽然可以改善数据局部性，但往往会带来较大的时间开销，严重影响端到端时间。 为此，许多并行重排序算法被提出。 通过实时重排序，同时实现高局部性和短重排序时间，大大减少通信延迟。
The neighbors of a vertex in a distributed system may exist in different nodes, and the frequent cache misses caused by the irregularity of the graph will lead to a large number of inter-core communications during parallel processing, which limits the overall operating efficiency. Although reorder can improve data locality, it often has a large time overhead, which seriously affects the end-to-end time. For this reason, many parallel reordering algorithms have been proposed. Simultaneously achieve high locality and short reordering time through real-time reordering, greatly reducing communication delays.

\textbf{a) Reorder for reducing communication latency}

1) RabbitOrder\cite{2016RabbitOrder}

2) ParallelRCM\cite{2017RCM}

\textbf{b) Comparisons of methods for reducing communication latency}
 
 \todo{time complexity O(n)}

%------------------------------------------------------------------
%%%%% 对比分析
%------------------------------------------------------------------
\subsection{Comparison and Analysis}

%之前，我们根据优化目标详细介绍了各种预处理方法的机制。 可以看出，针对不同的算法模型、图规模和执行设备采用不同的预处理方法，不同的预处理方法提供执行优化。 在这里，我们将在算法模型和硬件加速方面做一个全面的总结和对比。
Previously, we introduce the mechanism of various preprocessing methods in detail according to the optimization target. It can be seen that different preprocessing methods are used for different algorithm models, graph scales, and execution devices, different preprocessing methods to provide execution optimization. Here, we will give a comprehensive summary and comparison in algorithm model and hardware acceleration.

\noindent{\textit{A. Summary of preprocessing in algorithm optimization}}

%前文描述的预处理方法应用于模型的不同算法和执行步骤。 为了实现执行优化，一些预处理方法会导致信息丢失并影响计算结果。 因此，在选择方法时，需要根据模型机制在保证精度的同时，最大限度地提供优化。 在性能优化和精度损失之间存在权衡。
The preprocessing methods introduced before are applied to different algorithms and execution steps of the model. To achieve execution optimization, some preprocessing methods cause information loss and affect the computing results. Therefore, it is necessary to provide optimization to the maximum extent while ensuring accuracy according to the model mechanism when choosing methods. There is a trade-off between performance optimization and accuracy loss.

%-------------------------- preprocessing 模型应用 --------------------------------%
\begin{table*}[h]
\vspace{-0.15cm}  %调整表格与上文距离
\caption{Summary of preprocessing methods in algorithm optimization}
\vspace{-0.3cm}  %调整表格标题距离
\label{table:summary-algorithm}
\renewcommand{\arraystretch}{1.2}%调行距
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{Method} & Tradition & \multicolumn{2}{c|}{GNN}              & \multirow{2}{*}{Pipline} & \multirow{2}{*}{Accuracy}\\ 
\cline{2-4}
                        & Backbone  & \multicolumn{1}{c|}{Backbone} & phase &                          &  \\ 
\hline
Partition         & all       & GCN, GAT       & Train. \& Infer.     & offline \& online        &  no   \\
\hline
Sampling          &  -        & GCN, GAT       & Train.               & online                   &  loss  \\
\hline
Sparsification    & -         & GCN, GAT, GIN  & Train. \& Infer.     & online                   &  upgrade  \\
\hline
Reconstruction    & -         & GCN, GAT       & Train. \& Infer.     & online                   &  no   \\
\hline
Quantization      & -         & GCN, GAT       & Train. \& Infer.     & offline \& online        &  loss  \\
\hline
Data Reorder            & all       & GCN, GAT       & Train. \& Infer.     & offline \& online        &  no   \\
\hline
Blocking           & all       & GCN, GAT       & Infer.               & offline                  &  no   \\
\hline
\end{tabular}
\vspace{-0.15cm}  %调整表格与下文距离
\end{table*}

Due to the irregular structure of the graph, traditional graph computing has irregular execution behavior. GNN has two phases of graph aggregation and neural network transformation, with both regular and irregular execution behaviors. According to the different execution characteristics of traditional graph computing and GNN, different preprocessing methods are used for optimization.

\textit{Some preprocessing methods can be used for both tradition graph computing and GNN.} The Partiton method is used to divide large-scale input graphs. As the most common preprocessing method, it is suitable for almost all graph applications. For irregular storage access, a feasible optimization idea is to improve the locality of data access. Reorder improves access efficiency by placing frequently accessed data in close proximity and blocking optimizes access data flow through data partitioning.

\textit{Some preprocessing methods are only applicable to GNN.} Since GNN has a neural network transformation stage, the optimization methods commonly used in NN models can be extended to GNN, including sample, sparsification, and quantization. These methods can effectively reduce the amount of computation and achieve algorithm acceleration. Reconstruction reduces repeated aggregation and improves computational efficiency by merging shared neighbors. It is worth noting that most of the existing GNN preprocessing is only applicable to GCN and GAT models.

%Partition：大规模的图神经网络训练很难在单机上运行，所以需要parition将输入图分配给不同的节点进行训练。 图划分一般不会造成信息丢失。 对于每个顶点独立的mini-batch训练，partiton方法将一些顶点的邻居划分到其他节点中，影响了采样结果，但对准确率的影响很小。 图划分一般是离线的，不阻塞后续的数据训练。 针对大规模图数据的分割可能需要较长的计算时间，提出了一些启发式流采样来实现在线分割。
\textbf{Partition}: Large-scale graph neural network training is difficult to run on a single machine, so parition is required to assign the input graph to different nodes for training. Graph partitioning generally does not cause information loss. For the independent mini-batch training of each vertex, partiton method divides the neighbors of some vertices into other nodes which affects the sampling results, but the impact on accuracy is slight. Graph partition is generally offline and do not block subsequent data training. For the partiton of large-scale graph data may require a long computing time, some heuristic streaming sampling are proposed to achieve online partiton.

%Sample：对输入图进行采样得到mini-batch，相比full-batch的方式大大加快了采样的收敛速度。 由于并非所有顶点都用于训练 mini-batch，因此采样不可避免地会带来精度损失。 为此，分层采样 [faseGCN] [AS-GCN] [LADIES] 利用重要性采样技术来减少训练方差，而其他工作如 [cluster-GCN] [graphsaint] 添加特定机制以减少精度损失。 值得注意的是，采样是在线进行的，每次迭代都需要重采样。 对于大规模数据集，一些高复杂度的采样方法需要很长时间，这可能会阻塞计算管道。
\textbf{Sampling}: The input graph is sampled to obtain mini-batch, which greatly speeds up the convergence of sampling compared with full-batch manner. Since not all vertices are used to train the mini-batch, sampling inevitably brings loss of accuracy. To this end, layer-wise sampling \cite{2018FastGCN}\cite{2021AS-GCN}\cite{2019LADIES} utilizes importance sampling techniques to reduce training variance, while others works such as Cluster-GCN \cite{2019Cluster-GCN} and GraphSAINT \cite{2019graphsaint} add specific mechanisms to reduce accuracy loss.  It is worth noting that sampling is online and it is required each iteration. For large-scale datasets, some high-complexity sampling methods take a long time, which may block the computing pipeline.

%稀疏化：稀疏化在执行过程中丢弃多余的边，提高计算效率，缓解训练过程中的过度平滑问题。 由于增加了随机性，稀疏化方法可以提高准确性。 稀疏化是在线进行的。 启发式稀疏化执行速度很快，但只能产生局部最优。 基于边缘预测器稀疏化的算法更复杂，但它们可以更有效地解决过度平滑问题，这对于一些复杂的图模型至关重要。
\textbf{Sparsification}: Sparsification discards redundant edges during execution, improving computing efficiency and alleviating the over-smoothing problem in the training process. Due to the increased randomness, the sparsification method can improve the accuracy. Sparsification is performed online. Heuristic sparsification performs fast, but only yields local optima. Algorithms based on edge predictor sparsification are more complex, but they can solve the over-smoothing problem more effectively, which is essential for some complex graph models.

%重构：重构预先计算导致重复聚合的部分，以减少训练和推理过程中的冗余约简操作。 重构只是合并数据，不会造成信息丢失，不影响计算精度。 重建是轻量级的，它是在线执行的。
\textbf{Reconstruction}: Reconstruction calculate the part which lead to repeated aggregation in advance to reduce redundant reduction operations during training and inference. Reconstruction only merges data, so it does not cause information loss and does not affect computing accuracy. Reconstruction is lightweight and it performs online.

%量化：量化的核心思想是在训练过程中高精度模型很重要，但在推理阶段不需要高精度表示。 量化可以大大减少数据量，从而减少数据访问开销，实现整体加速。 一些方法通过特定的策略来减少精度损失。 SGQuant使用finetune提高精度，DegreeBased根据顶点的度数使用高精度和低精度的数据来减少高度顶点的误差累积。
\textbf{Quantization}: The core idea of quantization is that high-precision models are important during training, but high-precision representations are not required in the inference phase. Quantization can greatly reduce the data amount, thereby reducing data access overhead and achieving overall acceleration. Some methods reduce accuracy loss through specific strategies. SGQuant\cite{2020SGQuant} uses finetune to improve precision, and DegreeQuant\cite{2020DegreeQuant} uses high-precision and low-precision data according to the degree of vertices to reduce the error accumulation of high-degree vertices.

%reorder：Reorder 方法重新排列每个顶点的 ID，以改善数据局部性并降低缓存未命中率。 这种存储优化可用于训练和推理。 大多数重新订购方法都是离线的。 Gorder 和 Recall 等重量级重排序极大地利用了空间局部性，但计算复杂度非常高，并且对大型数据集进行重排序的成本很高。 为了减少重新排序时间，许多作品使用轻量级重新排序方法，包括 Rubik、H-GCN、GraphA、GCoD 等。
\textbf{Reorder}: Reorder methods rearrange the ID of each vertex to improve data locality and reduce the cache miss rate. This optimization for storage can be used for both training and inference. Most of the reorder methods are offline. Heavyweight reorder such as Gorder \cite{2016Gorder} and Recall \cite{2017Recall} have greatly exploited the spatial locality, but the computing complexity is very high, and cost expensive to reorder large datasets. To reduce the reorder time, many works use lightweight reorder methods, including Rubik, H-GCN \cite{2022H-GCN}, GraphA \cite{2022GraphA}, GCoD \cite{2022GCoD}, etc.

%阻塞：阻塞通过数据布局优化改进数据流访问的形式，从而增加数据的可重用性，提高存储带宽利用率。 出块方式都是离线的，难点在于如何选择最合适的块大小。 大多数设计长期需要手动调优，而SnF[]通过设计动态调优引擎实现了自动调优。
\textbf{Blocking}: Blocking improves the form of data flow access through data layout optimization, thereby increasing data reusability and improving storage bandwidth utilization. The blocking methods are all offline, and the difficulty lies in how to choose the most appropriate block size. Most designs long-time require manual tuning, and SnF \cite{2022SnF} realizes automaic tuning by designing a dynamically tuned engine.



\noindent{\textit{B. Summary of preprocessing in hardware acceleration}}

%图算法的执行依赖于硬件设备。 研究人员正在基于各种硬件平台优化图算法执行，以实现硬件加速。 在这些工作中，各种预处理方法被用来辅助算法执行。
The execution of graph algorithms depends on hardware devices. Researchers are optimizing graph algorithm execution based on various hardware platforms to achieve hardware acceleration. In these works, various preprocessing methods are used to assist algorithm execution.

%传统的图处理算法主要运行在 CPU 和 GPU 上。 此外，还有一些用于加速的定制设备。 执行传统的图处理算法有两个主要问题：1）如何划分大图以在多节点系统上运行。 2）如何减少频繁的冗余存储访问。 传统图计算中使用的预处理方法总结如表 x 所示。
1) The traditonal graph processing algorithms mainly run on CPU and GPU. Also, there are some customized devices used for acceleration. There are two main problems in executing traditional graph processing algorithms: 1) How to partition a large graph to run on a multi-node system. 2) How to reduce frequent redundant storage access. A summary of preprocessing methods used in traditional graph computing is shown in Table \ref{table:summary-hardware-tradition}.
%-------------------------- preprocessing 硬件应用 tradition --------------------------------%
\begin{table*}[h]
\vspace{-0.15cm}  %调整表格与上文距离
\caption{Summary of preprocessing methods for traditional graph computing in hardware acceleration}
\vspace{-0.3cm}  %调整表格标题距离
\label{table:summary-hardware-tradition}
\renewcommand{\arraystretch}{1.2}%调行距
\begin{tabular}{|l|l|l|l|p{8cm}|}
\hline
Method                                & Opt. Target                 & Scale                                 & Device & Works \\ 
\hline
\multirow{2}{*}{Partition}            & \multirow{2}{*}{\makecell[l]{Computing\\Communication}} & Multi-node                        & CPU    
& METIS \cite{1998METIS}, Pregel \cite{2010Pregel}, LDG \cite{2012LDG}, Graphlab \cite{2012graphlab}, Fennel \cite{2014Fennel}, PowerGraph \cite{2012powergraph}, BalanceEdge \cite{2014BalanceEdgePartition}, DBH \cite{2014DBH}, NE \cite{2017NE}, Germini \cite{2016Gemini}      \\ \cline{4-5} 
                                      &                                                     &                                       & GPU   
& Tiger \cite{2018Tigr}, Enterprise \cite{2015Enterprise}       \\ 
\hline
\multirow{2}{*}{Reorder}              & \multirow{2}{*}{\makecell[l]{Storage\\Communication}}   & \multirow{2}{*}{\makecell[l]{Single \\ Multi-node}} & CPU    
& RCM \cite{2014ParallelRCM}\cite{2017RCM}, Gorder \cite{2016Gorder}, Recall \cite{2017Recall}, RabbitOrder \cite{2016RabbitOrder}, Cagra \cite{2017Cagra}, ReorderHC \cite{2018ReorderHC}\\\cline{4-5}
                                      &                                                     &                                       & Custom  
& GraphQ \cite{2019GraphQ}, GraphA \cite{2022GraphA}       \\ 
\hline
\multirow{2}{*}{Blocking}             & \multirow{2}{*}{Storage}                            & \multirow{2}{*}{\makecell[l]{Single \\ Multi-node}} & CPU    
& Graphchi \cite{2012graphchi}, TurboGraph \cite{2013TurboGraph}, GridGraph \cite{2015gridgraph}       \\ \cline{4-5}
                                      &                                                     &                                       & Custom   
& Graphicionado \cite{2016graphicionado}       \\ 
\hline
\end{tabular}
\vspace{-0.15cm}  %调整表格与下文距离
\end{table*}

%分区：分区用于具有CPU和GPU的多节点系统，其目的是负载平衡和减少通信。
%Reorder：通过数据重新排序可以降低缓存未命中率。 对于单节点系统，重新排序可以减少不必要的内存访问开销。 对于分布式系统，重新排序可以帮助改善数据局部性并降低节点之间的通信频率。
%Blocking：传统图计算主要使用Interval-shard来提高内存访问数据流。 使用这种方法，传统的图算法可以在内存空间有限的单机上运行良好。
\textbf{Partition}: Partition is used in multi-node systems with CPU and GPU, which aims to the load balance and reduce communication. 

\textbf{Reorder}: The cache miss rate can be reduced through data reorder.  For a single-node system, reorder can reduce unnecessary memory access overhead. For a distributed system, reorder can help improve data locality and reduce communication frequency between nodes.

\textbf{Blocking}: Traditional graph computing mainly uses Interval-shard to improve memory access data flow. Using this method, traditional graph algorithms can run well on a single machine with limited memory space.

2) Researchers use CPUs, GPUs, or customized accelerators to execute GNN algorithms. There are 3 main problems in GNN execution: 1) How to partition large graph-scale graph input to run on multi-node systems. 2) How to reduce a large number of irregular storage accesses. 3) How to reduce the amount of data. The preprocessing methods used in GNN are summarized in Table \ref{table:summary-hardware-GNN}.
%-------------------------- preprocessing 硬件应用 GNN --------------------------------%
\begin{table*}[h]
\vspace{-0.15cm}  %调整表格与上文距离
\caption{Summary of preprocessing methods for GNNs in hardware acceleration}
\vspace{-0.3cm}  %调整表格标题距离
\label{table:summary-hardware-GNN}
\renewcommand{\arraystretch}{1.2}%调行距
\begin{tabular}{|l|l|l|l|p{7cm}|}
\hline
Method                          & Opt. Target                                         & Scale                                 & Device & Works \\ 
\hline
\multirow{3}{*}{Partition}  & \multirow{3}{*}{\makecell[l]{Computing\\Communication}} & \multirow{3}{*}{Multi-node}           & CPU    
& DistDGL \cite{2020DistDGL}, Dorylus \cite{2021Dorylus}, DistGNN \cite{2021DistGNN}      \\ \cline{4-5} 
                                &                                                     &                                       & GPU    
& PCGCN \cite{2020PCGCN},  PaGraph \cite{2020PaGraph}, Dorylus \cite{2021Dorylus}, PipeGCN \cite{2022PipeGCN}, BNS-GCN \cite{2022BNS-GCN}, Neugraph \cite{2019Neugraph}  \\\cline{4-5} 
                                &                                                     &                                       & Custom   
& Multi-FPGA-GNN \cite{2020Multi-FPGA-GNN}       \\ 
\hline
\multirow{2}{*}{Sampling}       & \multirow{2}{*}{\makecell[l]{Computing\\Storage}}   & \multirow{2}{*}{\makecell[l]{Single\\Multi-node}} & CPU    
& DistDGL \cite{2020DistDGL}       \\ \cline{4-5} 
                                &                                                     &                                       & GPU    
& PCGCN \cite{2020PCGCN}, PaGraph \cite{2020PaGraph}, Neugraph \cite{2019Neugraph}, GraphSage \cite{2017graphsage}, PinSage \cite{2018PinSage}, FastGCN \cite{2018FastGCN}, Cluster-GCN \cite{2019Cluster-GCN}, GraphSAINT \cite{2019graphsaint}        \\
\hline
\multirow{3}{*}{Sparsification} & \multirow{3}{*}{\makecell[l]{Computing\\Storage}}  & \multirow{3}{*}{\makecell[l]{Single\\Multi-node}}  & CPU    
& FastGAT \cite{2020FastGAT}, GLT \cite{2021GLT}      \\ \cline{4-5}
                                &                                                     &                                       & GPU    
& DropEdge \cite{2020DropEdge}, FastGAT \cite{2020FastGAT}, GLT \cite{2021GLT}       \\ \cline{4-5} 
                                &                                                     &                                       & Custom   
& DyGNN \cite{2021DyGNN}       \\ 
\hline
\multirow{3}{*}{Reconstruction} & \multirow{3}{*}{\makecell[l]{Computing\\Storage}}  & \multirow{3}{*}{\makecell[l]{Single\\Multi-node}}  & CPU    
& I-GCN \cite{2021I-gcn}       \\ \cline{4-5}
                                &                                                     &                                       & GPU   
& Redundancy-Free \cite{2020Redundancy-free}, I-GCN \cite{2021I-gcn}       \\ \cline{4-5} 
                                &                                                     &                                       & Custom   
& GcnInference \cite{2020GcnInference}, GraphACT \cite{2020GraphACT}       \\ 
\hline
\multirow{3}{*}{Quantization}   & \multirow{3}{*}{\makecell[l]{Computing\\Storage}}  & \multirow{3}{*}{\makecell[l]{Single\\Multi-node}}  & CPU    
& SGQuant \cite{2020SGQuant}, DegreeQuant \cite{2020DegreeQuant}       \\ \cline{4-5}
                                &                                                     &                                       & GPU    
& SGQuant \cite{2020SGQuant}, DegreeQuant \cite{2020DegreeQuant}, EXACT \cite{2021EXACT}, Bi-GCN \cite{2021Bi-GCN}, BiFeat \cite{2022BiFeat}, DBQ \cite{2022DBQ}  \\ \cline{4-5} 
                                &                                                     &                                       & Custom   
& FPGAN \cite{2020FPGAN}       \\ 
\hline
\multirow{3}{*}{Reorder}    & \multirow{3}{*}{\makecell[l]{Storage\\Communication}}   & \multirow{3}{*}{\makecell[l]{Single\\Multi-node}}  & CPU    &       \\ \cline{4-5}
                                &                                                     &                                       & GPU    
& GNNTiering \cite{2022GNNTiering}       \\ \cline{4-5} 
                                &                                                     &                                       & Custom 
& GcnInference \cite{2020GcnInference}, Rubik \cite{2021rubik}, H-GCN \cite{2022H-GCN}, GCoD \cite{2022GCoD}       \\ 
\hline
\multirow{2}{*}{Blocking}       & \multirow{2}{*}{Storage}                            & \multirow{2}{*}{\makecell[l]{Single\\Multi-node}} & GPU    
& Neugraph \cite{2019Neugraph}       \\ \cline{4-5}
                                &                                                     &                                       & Custom   
& HyGCN \cite{2020HyGCN}, AWB-GCN \cite{2020awbgcn}, GCNAX \cite{2021GCNAX}, EnGN \cite{2020EnGN}, SnF \cite{2022SnF}       \\ 
\hline
\end{tabular}
\vspace{-0.15cm}  %调整表格与下文距离
\end{table*}

%分区：图形分区广泛用于 CPU 和 GPU 集群上的 GNN 训练。 图划分有两个目的：一是尽可能将顶点和边均匀分布到不同的节点上，实现负载均衡，提高计算效率； 另一种是通过分区来改善数据局部性，以减少节点之间的通信开销。
%sample：GNN 训练的高内存占用使得 GNN 很难在内存受限的设备上运行，这严重限制了 GNN 的可扩展性。 mini-batch训练每次只需加载一个mini-batch数据到内存空间，大大缓解了内存压力。 同时，mini-batch 训练加快了收敛速度，降低了整体的计算量。
%稀疏化：稀疏化消除了冗余数据，因此可以有效缓解存储压力，减少不必要的计算。 与采样一样，稀疏化方法具有通用性，已应用于基于各种硬件平台的工作中。
%重构：重构通过预先合并公共边来减少重复聚合，大大减少了冗余计算。 重构过程的开销很短，可以在多种设备中使用。 尤其是在定制的加速架构中，重构具有很强的加速效果。
%量化：量化是一种广泛使用的通用压缩方法，可以有效减少数据量。 对于一般的 CPU 和 GPU 平台，量化大大缓解了缓存压力。 此外，一些定制的加速架构将 GNN 中的矩阵乘法转换为位移运算，从而大大降低了计算复杂度。
%重新排序：重新排序方法在一些定制的 GNN 加速器中受到青睐，它利用数据局部性来提高访问带宽利用率。
%分块：最常见的分块方法是分块技术，用于优化矩阵乘法运算。 作为优化 GPU 数据流的经典方法，它被用在一些使用 GPU 的 GNN 训练工作中。 针对稀疏矩阵乘法的优化适合加速器技术，tiling在定制架构中取得了很好的加速效果。

\textbf{Partition}: Graph partitioning is widely used in GNN training on CPU and GPU clusters. Graph partitioning has two purposes: one is to evenly distribute vertices and edges to different nodes as much as possible to achieve load balancing and improve computing efficiency; the other is to improve data locality through partitioning to reduce communication overhead between nodes.

\textbf{Sampling}: The high memory usage of GNN training makes it difficult for GNN to run on memory-constrained devices, which severely limits the scalability of GNN. The mini-batch training only needs to load one mini-batch of data into the memory space each time, which greatly relieves the memory pressure. At the same time, mini-batch training speeds up the convergence speed and reduces the overall computational load.

\textbf{Sparsification}: Sparsification eliminates redundant data, so it can effectively alleviate storage pressure and reduce unnecessary computing. Like sampling, the sparsification method is versatile and has been applied in work based on various hardware platforms.

\textbf{Reconstruction}: Reconstruction reduces repeated aggregation by merging common edges in advance, which greatly reduces redundant calculations. The overhead of the reconstruction process is very short, and it can be used in a variety of devices. Especially, in the customized acceleration architecture, reconstruction has a strong acceleration effect.

\textbf{Quantization}: Quantization is a widely used general-purpose compression method that can effectively reduce the amount of data. For general CPU and GPU platforms, quantization greatly relieves cache pressure. Besides, some customized acceleration architectures convert the matrix multiplication in GNN into bitshift operations, which greatly reduces the computational complexity.

\textbf{Reorder}: The reorder method is favored in some customized GNN accelerators, which exploits data locality through to improve access bandwidth utilization.

\textbf{Blocking}: The most common blocking method is tiling technology, which is used to optimize matrix multiplication operations. As a classic method to optimize GPU data flow, it is used in some GNN training work using GPU. The optimization for sparse matrix multiplication is suitable for accelerator technology, and tiling has achieved good acceleration results in customized architectures.


==> old/evaluation.tex <==
\todo{omparison about 5 pages}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\begin{tabular}{@{}cccccccc@{}}
\toprule[1.5pt]
\multicolumn{3}{c}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}CATEGORY\\ Efficient Computing\end{tabular}}} & \multicolumn{2}{c}{Preprocessing Resource Overhead} & \multicolumn{3}{c}{Overall Effect}     \\ \cmidrule(l){4-8} 
\multicolumn{3}{c}{}                                                                                        & Memory Usage              & Prepro.Time             & Runtime      & Total Time   & Accuracy \\ \midrule
\multicolumn{2}{c}{\multirow{2}{*}{Baseline}}                                         & Cora                & 50.1\%                    & -                       & 4.80 ± 0.42s & 4.80 ± 0.42s (1.5$\times$) & 0.814    \\
\multicolumn{2}{c}{}                                                                  & Citeseer            & 60.5\%                    & -                       & 5.44 ± 0.30s & 5.44 ± 0.30s (1.5$\times$) & 0.711    \\ \midrule
\multirow{6}{*}{Sample}                    & \multirow{3}{*}{GraphSage}               & Cora                &                           &                         &              &              &          \\
                                           &                                          & Citeseer            &                           &                         &              &              &          \\
                                           &                                          & Reddit              &                           &                         &              &              &          \\ \cmidrule(l){2-8} 
                                           & \multirow{3}{*}{GraphSaint}              & Cora                &                           &                         &              &              &          \\
                                           &                                          & Citeseer            &                           &                         &              &              &          \\
                                           &                                          & Reddit              &                           &                         &              &              &          \\ \midrule
\multirow{6}{*}{Partition}                 & \multirow{3}{*}{METIS(PCGCN)}            & Cora                &                           &                         &              &              &          \\
                                           &                                          & Citeseer            &                           &                         &              &              &          \\
                                           &                                          & Reddit              &                           &                         &              &              &          \\ \cmidrule(l){2-8} 
                                           & \multirow{3}{*}{todo}                    & Cora                &                           &                         &              &              &          \\
                                           &                                          & Citeseer            &                           &                         &              &              &          \\
                                           &                                          & Reddit              &                           &                         &              &              &          \\ \midrule
\multirow{6}{*}{Sparsification}            & \multirow{3}{*}{todo}                    & Cora                &                           &                         &              &              &          \\
                                           &                                          & Citeseer            &                           &                         &              &              &          \\
                                           &                                          & Reddit              &                           &                         &              &              &          \\ \cmidrule(l){2-8} 
                                           & \multirow{3}{*}{todo}                    & Cora                &                           &                         &              &              &          \\
                                           &                                          & Citeseer            &                           &                         &              &              &          \\
                                           &                                          & Reddit              &                           &                         &              &              &          \\ \midrule
\multirow{6}{*}{Reconstruction}            & \multirow{3}{*}{I-GCN}                   & Cora                &                           &                         &              &              &          \\
                                           &                                          & Citeseer            &                           &                         &              &              &          \\
                                           &                                          & Reddit              &                           &                         &              &              &          \\ \cmidrule(l){2-8} 
                                           & \multirow{3}{*}{todo}                    & Cora                &                           &                         &              &              &          \\
                                           &                                          & Citeseer            &                           &                         &              &              &          \\
                                           &                                          & Reddit              &                           &                         &              &              &          \\ \midrule
\multirow{6}{*}{compression}               & \multirow{3}{*}{SGQuant}                 & Cora                &                           &                         &              &              &          \\
                                           &                                          & Citeseer            &                           &                         &              &              &          \\
                                           &                                          & Reddit              &                           &                         &              &              &          \\ \cmidrule(l){2-8} 
                                           & \multirow{3}{*}{DegreeQuant}             & Cora                &                           &                         &              &              &          \\
                                           &                                          & Citeseer            &                           &                         &              &              &          \\
                                           &                                          & Reddit              &                           &                         &              &              &          \\ \midrule
\multirow{6}{*}{rearrangement}             & \multirow{3}{*}{}                        & Cora                &                           &                         &              &              &          \\
                                           &                                          & Citeseer            &                           &                         &              &              &          \\
                                           &                                          & Reddit              &                           &                         &              &              &          \\ \cmidrule(l){2-8} 
                                           & \multirow{3}{*}{}                        & Cora                &                           &                         &              &              &          \\
                                           &                                          & Citeseer            &                           &                         &              &              &          \\
                                           &                                          & Reddit              &                           &                         &              &              &          \\ \bottomrule[1.5pt]
\end{tabular}
\end{table}

==> old/future-old.tex <==
%在本节，我们讨论预处理面临的挑战和未来的研究方向。 尽管预处理方法在各种图处理加速工作中取得了成功，但由于算法和设备的一些因素，仍然存在着挑战。
In this section, we discuss challenges and future directions of graph preprocessing. Although preprocessing methods have achieved success in various graph processing acceleration efforts, challenges are still existing due to some factors of algorithms and devices.

%------------------------- 挑战
\subsection{Challenges in Graph Preprocessing}

%首先，随着数据规模的增大，预处理所需的时间开销愈发不可忽视。一些启发式的方法降低预处理时间，但相比于复杂的预处理方法，这些启发式方法的优化效果相对较差甚至会影响精度。其次，为了降低数据量，预处理方法不可避免的会造成精度损失。虽然很多改进的方法被提出用于降低精度损失，但仍需要在精度和优化效果进行权衡。第三，现有的GNN方法局限于优化浅层GCN模型，且大多针对同构图。目前，异构图模型成为新的研究趋势，对于异构图的预处理是一项值得研究的工作。接下来我们讨论预处理的一些潜在的未来方向。
Currently, there are three main challenges. First, as the scale of data increases, the time overhead required for preprocessing are becoming more non-negligible. Some heuristics reduce preprocessing time, but compared to complex preprocessing methods, these heuristics are relatively poorly optimized and even affect accuracy. Second, in order to reduce the amount of data, preprocessing methods such as quantization and sampling inevitably cause precision loss. Although many improved methods have been proposed to reduce the loss of accuracy, there is still a trade-off between accuracy and optimization effect. Third, existing GNN methods are mostly used in isomorphic graphs. Recently, the heterogeneous graph model has become a new research trend, and the preprocessing of heterogeneous graphs is a work worth studying. 


\subsection{Future Directions}
Next we discuss some potential future directions for preprocessing.

$\bullet$ \textbf{Pipeline-friendly Preprocessing}

%随着数据规模的爆炸式增长和模型复杂度的增加，预处理的开销变得更大。 更好的加速方法往往对应于预处理算法的复杂度增加。 以重新排序为例，Gorder 和 Recall 等重量级方法可以充分利用数据局部性。 然而，大多数加速作品如[GCNinference] [Rubik] [H-GCN] 仍然使用轻量级的RCM或LSH算法。 是因为Gorder、Recall等方法的时间复杂度很高，导致流水线停顿。 而如果经过长时间预处理的数据可以多次重复使用，则预处理时间可以与后续算法执行时间重叠。 为了达到最好的加速效果，在研究加速时需要综合考虑后续的执行时间和预处理开销，慎重选择最佳的预处理方式。
As the data scale explodes and the model complexity increases, the overhead of preprocessing becomes larger. A better acceleration method often corresponds to an increasing complexity of the preprocessing algorithm. Taking reorder as an example, heavyweight methods such as Gorder and Recall can exploit data locality adequately. However, most acceleration works such as works \cite{2020GcnInference}\cite{2021rubik}\cite{2022H-GCN} still use lightweight RCM or LSH algorithms. It is because the time complexity of methods such as Gorder and Recall is very high, which leads to the stall of the pipeline. While, if the data that has been preprocessed for a long time can be reused many times, the preprocessing time can be overlapped by the subsequent algorithm execution time. In order to achieve the best acceleration, it is necessary to comprehensively consider subsequent execution time and preprocessing overhead when researching acceleration, and carefully select the best preprocessing method.

$\bullet$ \textbf{Accuracy-friendly Preprocessing}

%量化、采样等预处理方法可以大大降低存储需求，提高计算速度，但不可避免地会带来误差，影响最终的计算精度。 为了减少方差，一些方法如【SGQuant】[DegreeQuant]，使用特殊的机制来减少精度损失，但会需要更多的内存空间。 EXACT【】通过投影减少精度损失，但需要额外的缓冲区来存储中间结果。 因此，需要综合考虑精度损失和优化效果，做出权衡。
Preprocessing methods such as quantization and sample can greatly reduce storage requirements and improve computing speed, but inevitably bring errors and affect the final computing accuracy. In order to reduce the variance, some methods such as SGQuant \cite{2020SGQuant} and DegreeQuant \cite{2020DegreeQuant}, use special mechanisms to reduce the loss of precision, but will require more memory space. EXACT \cite{2021EXACT} reduces precision loss through projection, but requires additional buffers to store intermediate results. Therefore, it is necessary to comprehensively consider the loss of accuracy and the optimization effect, and make a trade-off.

$\bullet$ \textbf{General-framework of Preprocessing}

%为了达到更好的优化效果，往往会采用多种预处理方法。 [DistDGL] [PCGDCN]等分布式GNN训练作品首先将输入图划分为子图，然后对子图进行采样进行训练。 在GcnInference[]的预处理过程中，首先进行重构消除冗余，然后对重构后的图数据进行重新排序。 SnF[]基于分块进行数据流优化，然后执行graphsage等图采样模型。 因此，研究多种方法的适应性和冲突，探索多种预处理方法的通用可配置框架是一项有意义的工作。
To achieve better optimization, it often use a variety of preprocessing methods. Distributed GNN training works such as work \cite{2020DistDGL}\cite{2020PCGCN} first divide the input graph into subgraphs and then sample the subgraphs for training. In the preprocessing process of work \cite{2020GcnInference}, it first executes reconstruction to eliminate redundancy, then reorder the reconstructed graph data. SnF \cite{2022SnF} performs data flow optimization based on blocking, and then executes graph sampling models such as GraphSage. Therefore, it is a meaningful work to study the adaptability and conflict of multiple methods and to explore a general configurable framework for multiple preprocessing methods.

$\bullet$ \textbf{Preprocessing for Heterogeneous Graph}

%最近，异构图的研究呈现出越来越大的趋势，作品[HCCN]、[hetero]、[hetero-gate]、[hetersurvey]都是最近的作品。 异构图通常包括不同类型的边和顶点[元路径]，现有的面向同构图的预处理工作不能直接应用于异构图模型。 异构图的预处理方法只有几种[][]。 因此，针对异构图加速设计具体的预处理方法具有重要的研究价值。
Recently, research on heterogeneous graphs has shown a growing trend, works \cite{2020Hgcn}\cite{2022sybilflyover-hetero}\cite{2022heteroGNNgate}\cite{2022survey-hetero} are recent works. Heterogeneous graphs usually include different types of edges and vertices \cite{2018meta-path}, existing preprocessing works oriented to isomorphic graphs cannot be directly applied to heterogeneous graph models. There are only a few preprocessing methods of heterogeneous graphs \cite{2019HetGNN}\cite{2020HGSampling}. Therefore, it is of great research value to design specific preprocessing methods for heterogeneous graph acceleration.

==> old/introduction_old.tex <==
%---------------------------------------------------------------------------------------------
%%%% 图是一种数据结构，它使用顶点和边对对象之间的关系进行建模。在现实世界中，许多类型的数据可以使用图结构来表示，社交网络是最常见的例子之一，如图1(a)所示，facebook网络被抽象为图。图处理算法因其从图数据中提供的有价值的见解而受到了极大的关注，大致包含两种类型：a.传统图处理算法，如Breadth First Search (BFS), PageRank (PR)等；b.图神经网络算法，如Graph Convolution Networks (GCN), Graph Auto-Encoder (GAE)等。图处理算法在
%---------------------------------------------------------------------------------------------


%---------------------------------------------------------------------------------------------
%%%% 图：基本定义和特点（数据结构，不规则特性）
%---------------------------------------------------------------------------------------------
Graphs are a type of data structure that model relationships between objects using vertices and edges. In real world, many types of data can be represented using graph structures with social networks \cite{2020GTinCSandSN} being one of the most common examples. Figure \ref{fig:facebook} provides visual representation: (a) depicts a friend network in Facebook, (b) abstracts this social network as a graph, with vertices representing users and edges representing their relationships, and (c) demonstrates the topology of image data and text sequences. A comparison between (b) and (c) reveals that the graph topology is irregular, with non-uniform connections between vertices, setting it apart from grid-structured images and linear-structured text sequences. Nowadays, graphs find extensive application as effective data representations in diverse domains, including e-commerce networks \cite{2020recommendGNN}, molecular structures \cite{2021protein}, and traffic networks \cite{2020trafficgman}, etc.

\begin{figure}[ht]
    \centering
    \vspace{-0.2cm}  %调整图片与上文的垂直距离
    \setlength{\abovecaptionskip}{0.2cm}     %调整图片标题与图距离
    \setlength{\belowcaptionskip}{-0.2cm}   %调整图片标题与下文距离
    \includegraphics[width=\textwidth]{fig-introduction/facebook.eps}
    \caption{Graph abstracted from social networks vs. Image and Text: (a) Friends Network in Facebook; (b) Graph abstracted from the Friends Network; (c) Topology of Image and Text sequence.}
    \label{fig:facebook}
\end{figure}

%---------------------------------------------------------------------------------------------
%%%% 图应用，图算法
% 图处理算法因其从图数据中提供的有价值的见解而受到了极大的关注
%---------------------------------------------------------------------------------------------
Graph processing algorithms have garnered significant attention due to the valuable insights they offer from graph data, which can be broadly categorized into two types: a. Traditional Graph Algorithms, including Breadth First Search (BFS), PageRank (PR), Single Source Shortest Paths (SSSP), Single Source Widest Paths (SSWP), etc. These algorithms are applied to tackle various problems, such as social network recommendation \cite{2019rankingPagerank}, knowledge graph analysis \cite{2019bfsknowledgeGraph}, etc. b. Graph Neural Network (GNN) algorithms, such as Graph Convolution Networks (GCN), Graph Auto-Encoder (GAE), Graph Recurrent Networks (GRN), etc. These algorithms find applications in protein prediction \cite{2021protein-predict}, image recognition \cite{2019imagemulti}, etc. To handle the growing volume of graph data, graph processing applications have been widely deployed in various data centers, making them one of the most popular applications in the field. Figure \ref{fig:application} shows various application scenarios where graph processing algorithms are utilized.

\begin{figure}[ht]
    \centering
    \vspace{-0.2cm}  %调整图片与上文的垂直距离
    \setlength{\abovecaptionskip}{0.2cm}     %调整图片标题与图距离
    \setlength{\belowcaptionskip}{-0.2cm}   %调整图片标题与下文距离
    \includegraphics[width=\textwidth]{fig-introduction/application.eps}
    \caption{Applications of Graph Processing Algorithms}
    \label{fig:application}
\end{figure}

%---------------------------------------------------------------------------------------------
%%%% 图应用的执行行为：
%    由于模型和输入数据的差异，图处理算法具有不同的执行行为。 传统图算法的执行行为主要由输入数据决定，由于图的非结构化和分布不均匀，具有不规则的特征。 图3(a)显示了BFS的计算过程，可以发现每次迭代访问的顶点数取决于图的拓扑结构。 
%    GNN 算法融合了传统图处理和神经网络的执行过程，使得不规则和规则行为并存[28]。 图3(b)展示了GCN的计算过程，包括信息收集的聚合阶段和神经网络变换的组合阶段
%---------------------------------------------------------------------------------------------
Graph processing algorithms have different execution behaviors due to differences in models and input data. The execution behavior of traditional graph algorithms, which is mostly decided by input data, owing irregular characteristics due to the unstructured and uneven distribution of graph. Figure 3 (a) shows the computing process of BFS, which can be found that the number of vertices accessed per iteration depends on graph topology. GNN algorithms integrate the execution process of both tradition graph processing and neural network, making irregular and regular behaviors coexist \cite{2021lihansurvey}. Figure 3 (b) shows the computing process of GCN, which consists of aggregation stage of information collection and combination stage of neural network transformation.

\begin{figure}[ht]
    \centering
    \vspace{-0.2cm}  %调整图片与上文的垂直距离
    \setlength{\abovecaptionskip}{-0.3 cm}     %调整图片标题与图距离
    \setlength{\belowcaptionskip}{-0.2cm}   %调整图片标题与下文距离
    \includegraphics[width=\textwidth]{fig-introduction/bfs.eps}
    \caption{Examples of the computing process of Traditional Graph Algorithms and GNNs: (a) Traversal process of Breadth First Search (BFS); (b) Each iteration of Graph Convolution Network (GCN) first performs an aggregate operation to gather vertex information and then performs a combine operation for neural network transformation.}
    \label{fig:bfs}
\end{figure}

%---------------------------------------------------------------------------------------------
%%%% 图处理应用3个挑战：
%     首先，图处理算法的不规则执行行为限制了计算和内存访问效率。 大量的随机内存访问导致带宽利用率低，这通常成为限制性能的瓶颈。 
%     其次，图数据的爆发式增长给计算和存储带来了巨大的压力。 虽然分布式系统用于部署大规模图处理算法，但存在负载平衡和通信开销问题。 
%     第三，应用场景和设备对时间和吞吐量带来特殊要求。在某些情况下，数据需要实时更新，这种时间敏感的任务很容易达到无法接受的运行时间。 在其他一些情况下，设备上的资源有限，因此很难运行大规模算法。
%---------------------------------------------------------------------------------------------
However, it is discovered that graph processing applications are facing the following \textbf{three challenges}. First, \textbf{the irregular execution behaviors of graph processing algorithms} limits computing and memory access efficiency. Large amounts of random memory access leads to low bandwidth utilization, which usually becomes the bottleneck limiting performance. Second, \textbf{the explosive increasing of graph data} poses great pressure on computing and storage. Though distributed systems are used to deploy large scale graph processing algorithms, there are load balance and communication overhead issues. Third, \textbf{application scenarios and equipments bring special requirements for time and throughput.} In some cases, data need real-time update, such time-sensitive tasks can easily achieve unacceptable running time. In some other cases, resources on devices are limited so that it hard to run large scale algorithms. 

%---------------------------------------------------------------------------------------------
%%%% 现有survey：
%    为了应对上述挑战，近年来越来越多的工作致力于图处理执行优化的研究，力求提高图处理算法的执行效率。 一些文献总结和回顾了这些加速工作，我们在表 x 中对其进行了简要介绍。 
%    可以看出，图处理执行在算法和硬件上都进行了优化。 在算法方面，研究人员通过优化图形模型或调整输入数据模式来提高计算效率。 在硬件方面，研究人员设计高效的图算法执行框架或定制加速器来提高硬件执行效率。 
%    在这些加速工作中，各种预处理方法被广泛使用，然而，很少有工作关注图预处理的开销和执行效果。这是因为用有限数量的图数据执行预处理需要的时间很少，同时离线预处理的一次性成本可以被后续的图处理算法的多次迭代所覆盖。
%---------------------------------------------------------------------------------------------
\begin{table*}[h]
\vspace{-0.15cm}  %调整表格与上文距离
\caption{Surveys about graph processing acceleration works}
\vspace{-0.3cm}  %调整表格标题距离
\label{table:survey}
\begin{tabular}{|c|p{3cm}|p{10cm}|}
\hline
\textbf{Domain} & \textbf{Survey (Year)}    & \textbf{Contribution}    \\
\hline
\multirow{3}{*}{Hardware} 
& Graph processing on GPUs: A survey \cite{2018GraphGPUSurvey} (2018) 
& A survey of graph processing key issues on GPUs. \par $\bullet$ Summarize the state-of-the-art research on GPU-based graph processing. \par $\bullet$ Analyze the existing challenges: data layout, memory access pattern, workload mapping, and specific GPU programming. \par $\bullet$ Explore the research opportunities for future works.         \\
\cline{2-3}
& Scalable Graph Processing Frameworks: A Taxonomy and Open Challenges \cite{2018SurveyScalable} (2018)
& A survey of scalable graph processing systems. \par $\bullet$ Propose a taxonomy of graph processing systems and map existing works. \par $\bullet$ Analyze the diversity of in-memory and distributed framwork in programming and computation models and runtime. \par $\bullet$ Discuss the bottlenecks and future directions of large graph processing systems. \\
\cline{2-3}
& Survey on Graph Neural Network Acceleration: An Algorithmic Perspective \cite{liu2022survey} (2022)  & A survey of GNN acceleration methods from the algorithmic perspective. \par $\bullet$ Provide a taxonomy of GNN acceleration method. \par $\bullet$ Compare the efficiency and characteristics of these methods. \par $\bullet$ Suggest some promising prospects: acceleration for dynamic graphs, hardware-friendly algorithms, algorithm and hardware co-design. \\
\hline
\multirow{2}{*}{Algorithm}
& Computing graph neural networks: A survey from algorithms to accelerators \cite{2021GNNAlgToAccSurvey} (2021) 
& A survey of acceleration methods of GNN. \par $\bullet$ Provide a thorough review of GNN research from the perspective of computation. \par $\bullet$ Review the GNN algorithms and summarize the implementation of different GNN algorithm variants. \par $\bullet$ Presents the future directions of GNN acceleration: software-hardware co-design, graph awareness, communication-centric design. \\
\cline{2-3}
& Sampling methods for efficient training of graph convolutional networks: A survey \cite{2021liu-sampling-survey} (2021) 
& A systematic survey of sampling methods. \par $\bullet$ Categorize sampling methods based on the sampling mechanisms. \par $\bullet$ Present a detailed comparison within each category. \par $\bullet$ Suggest some potential directions of sampling: variance reduction and elimination, co-ordination with experimental platforms, hardware-friendly sampling, heterogeneous graph sampling, sampling in deep models.\\
\hline
\end{tabular}
\vspace{-0.5cm}  %调整表格与下文距离
\end{table*}

To meet the challenges above, recent years have seen increasing works devoted to study graph processing execution optimization, striving to improve the execution efficiency of graph processing algorithms. Some literature summarizes and reviews these acceleration works, which we briefly introduce in Table \ref{table:survey}. It can be seen that graph processing execution has been optimized in both algorithms and hardware. In algorithm ways, researchers optimize graph models or adjust input data patterns to improve computing efficiency. In hardware ways, researchers design efficient graph algorithm execution frameworks or customize accelerators to improve hardware execution efficiency. In these acceleration works, various preprocessing methods are widely used, such as sampling, reorder, etc. However, few works focus on the overhead and execution effects of graph preprocessing. This is because the preprocessing executing with limited amount of graph data requires little time, meanwhile the one-time cost of offline preprocessing can be overlapped by the subsequent multiple iterations of graph processing algorithms.

%---------------------------------------------------------------------------------------------
%%%% 预处理定义：
%    在这里，我们给出图预处理的解释——在图处理算法正式执行之前的过程，其中转换图表示或数据表示以辅助图处理执行加速。 
%    例如work[]通过采样降低计算复杂度，work[]通过重排提高存储访问效率等，这些都会在后面的章节中详细介绍。 
%    预处理主要帮助三个方面： 加速图形应用程序的执行。 b. 减少计算和存储资源开销。 C。 满足资源受限的设备算法运算需求。
%---------------------------------------------------------------------------------------------
Here, we give our \textbf{explanation of graph preprocessing}: the process before the formal execution of graph processing algorithms, in which transforming the graph representation or data representation to assist graph processing execution acceleration. For example, work \cite{2017graphsage}\cite{2018FastGCN}\cite{2019graphsaint}\cite{2019Cluster-GCN} reduce the computational complexity by sampling, work \cite{2016Gorder}\cite{2016RabbitOrder}\cite{2018ReorderHC}\cite{2021rubik}\cite{2022H-GCN} improve storage access efficiency by reorder, etc, all of which will be introduced in detail in the following sections. Preprocessing mainly helps in three aspects: a. Accelerate the execution of graph applications. b. Reduce computing and storage resource overhead. c. Meet the needs of resource-constrained device algorithm operations.

%---------------------------------------------------------------------------------------------
%%%% 预处理开销：
%    预处理开销变得不可忽略，这基于两个原因：一是图数据的爆炸式增长，导致预处理时间急剧增加。 二是图数据的实时更新，需要持续进行快速的在线预处理。
%    在工作[Gorder]中，大数据集Twitter的图重新排序需要1.5小时，而PageRank 100次迭代的运行时间只需要13.65分钟。 如果输入图不能多次重复使用，图重新排序得不偿失。 工作[sample survey]基于采样方法训练了一个两层GCN，其中模型Cluster-GCN和FastGCN具有非常相近的采样和训练运行时间。 Work【Adaptive sparse tiling】通过tiling加速稀疏矩阵乘法（SpMM）的运算，而tiling时间是SpMM计算时间的0~5倍。
%    表 x 显示了两层 GCN 训练的预处理时间和训练时间比率。 可以看出，预处理时间占整体训练时间的比例很高，因此减少预处理开销有助于提高整体执行效率。 然而，还没有文献对图预处理进行系统的分析和总结。
%---------------------------------------------------------------------------------------------
The \textbf{preprocessing overhead} is becoming non-negligible for two reasons: One is the explosive increase of graph data, which leads to the preprocessing time increase dramatically. Two is the real-time update of graph data, which requires to execute fast online preprocessing continuously. In work \cite{2016Gorder}, the graph reorder of large dataset Twitter takes 1.5 hours, while the running time of PageRank for 100 iterations only takes 13.65 minutes. If the input graph cannot be reused many times, the graph reorder is not worth the loss. The work \cite{2021liu-sampling-survey} trains a two-layer GCN based on the sampling method, in which model Cluster-GCN \cite{2019Cluster-GCN} and GraphSAINT \cite{2019graphsaint} have very close runtime of sampling and training. Work \cite{2019AdaptiveTilingSpMM} accelerate the operation of sparse matrix multiplication (SpMM) through tiling, while the tiling time is 0~5 times the calculation time of SpMM. Table \ref{table:preprcessing-time} shows the preprocessing time and training time ratio of a two-layer GCN training. It can be seen that the preprocessing time occupies a high ratio of the overall training time, so reducing the preprocessing overhead helps to improve the overall execution efficiency. However, there is no literature that systematically analyzes and summarizes graph preprocessing.

\begin{table*}[h]
\vspace{-0.15cm}  %调整表格与上文距离
\caption{Preprocessing and training time ratio of a two-layer GCN}
\vspace{-0.3cm}  %调整表格标题距离
\label{table:preprcessing-time}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Preprocessing Method} & \textbf{Model} & \textbf{Dataset} & \textbf{Preprocessing} & \textbf{Training} & \textbf{Pre./Training}    \\
\hline
\multirow{4}{*}{Sampling}
& \multirow{2}{*}{GraphSage \cite{2017graphsage}}
    & PPI      & 27.08\% & 72.92\% & 0.37 \\
    \cline{3-6}
    & & Reddit & 29.37\% & 70.63\% & 0.42 \\
    \cline{2-6}
& \multirow{2}{*}{GraphSAINT-edge \cite{2019graphsaint}}
    & PPI      & 56.08\% & 43.92\% & 1.28 \\
    \cline{3-6}
    & & Reddit & 29.86\% & 70.14\% & 0.43 \\
\hline
\multirow{3}{*}{Sparsification} 
& \multirow{3}{*}{DropEdge \cite{2020DropEdge}}
    & Cora       & 36.05\% & 62.07\% & 0.49 \\
    \cline{3-6}
    & & Citeseer & 67.83\% & 32.17\% & 2.11 \\
    \cline{3-6}
    & & Pubmed   & 68.45\% & 32.55\% & 2.10 \\
\hline
\end{tabular}
\vspace{-0.15cm}  %调整表格与下文距离
\end{table*}

%---------------------------------------------------------------------------------------------
%%%% 贡献：在本文中，我们从算法和硬件的角度对图预处理方法进行了系统的归纳和分析。 据作者所知，这是对图预处理方法的首次全面调查。 我们的贡献如下：
%       Review：我们从算法的角度总结和回顾了现有的预处理方法，按照核心机制总结了7种主要的图预处理方法:xxxxxxx
%       Taxonomy：我们分析了图形处理加速在硬件层面的挑战，并根据优化目标提出了我们的分类法：高效计算、高效存储和高效通信。
%       Comparison：我们根据分类法详细介绍了预处理方法，并比较了这些方法的适用性和成本。
%       Discuss：我们讨论了图预处理的挑战和未来的研究方向。
%---------------------------------------------------------------------------------------------
In this paper, we provide a systematical induction and analysis of graph preprocessing methods from both algorithmic and hardware perspectives. To the best of the authors' knowledge, this is the first comprehensive survey of graph preprocessing methods. Our contributions are as follows:

1) \textbf{Review}: We summarize and review the existing preprocessing method from the perspective of algorithms, and summarize 7 main graph preprocessing methods according to the core mechanism: partition, sampling, sparsification, reconstruction, quantization, reorder and blocking.

2) \textbf{Taxonomy}: We analyze the challenges for graph processing acceleration in hardware level, and propose our taxonomy according to the optimization targets: efficient computing, efficient storage, and efficient communication.

3) \textbf{Comparison}: We introduce the preprocessing methods in detail according to our taxonomy, and compare the applicability and cost of these methods.

4) \textbf{Discussion}: We discussed the challenges of graph preprocessing and future research directions.

%---------------------------------------------------------------------------------------------
%%%% 文章组织结构介绍
%    第二节介绍相关背景，首先介绍图表示和图算法，然后介绍现有的图预处理方法。最后阐述硬件层次面临的挑战，并提出我们的分类法。根据硬件优化目标，将预处理方法分为3类.
%    第三节详细阐述我们的分类法，并从多个方面对比分析。
%    第四节分析当前预处理的瓶颈并讨论未来的潜在方向
%    第五节进行总结。
%---------------------------------------------------------------------------------------------
The rest of this paper is organized as follows. We introduce background in Section \ref{background}. We first introduce graph representation and graph algorithms, then introduce existing graph preprocessing methods. Last, we describe challenges in hardware level and propose our taxonomy. According to the target of hardware optimization, graph preprocessing methods are classified into 3 categories. In Section \ref{category}, we elaborate our taxonomy in details and compare and analyze the methods in multiple aspects. In Section \ref{future}, we analyze the bottlenecks of graph preprocessing and discuss some potential directions. Finally, we conclude this paper in Section \ref{conclusion}.

%In Section \ref{evaluation}, we conduct experiments on typical methods to evaluate the effects and overhead of different preprocessing methods.





==> old/name.tex <==
\begin{table*}[h]
\vspace{-0.15cm}  %调整表格与上文距离
\caption{Surveys about graph processing acceleration and the GPP methods involved}
\vspace{-0.3cm}  %调整表格标题距离
\label{table:survey}
\centering
\begin{tabular}{|m{9cm}|c|c|}
\hline
\makecell[c]{\textbf{Survey (Year)}} & \textbf{Domain} & \textbf{GPP}\\ \hline
$\bullet$ Graph Processing on GPUs: A Survey (2018) \cite{2018GraphGPUSurvey} &  \makecell{TGC\\GPU} & \makecell{Partition\\Reorganization} \\ \hline

$\bullet$ Graph Processing on FPGAs: Taxonomy, Survey, Challenges (2019) \cite{2019GraphFPGASurvey} & \makecell{TGC\\FPGA} & \makecell{Partition\\Reorganization} \\ \hline

$\bullet$ A Survey on Graph Processing Accelerators: Challenges and Opportunities (2019) \cite{2019GraphAccSurvey} & \makecell{TGC\\ASIC \& FPFA \& PIM} & \makecell{Partition\\Reorder}\\ \hline

$\bullet$ Graph Processing and Machine Learning Architectures with Emerging Memory Technologies: A Survey (2021) \cite{2021graphMemorySurvey} & \makecell{TGC \& GNN \\ Memory} & \makecell{Reorganization}\\ \hline

$\bullet$ Thinking Like a Vertex: A Survey of Vertex-Centric Frameworks for Large-Scale Distributed Graph Processing (2015) \cite{2015ThinkingVertexSurvey} & \makecell{TGC \\ Distributed System} & \makecell{Partition\\Reorganization} \\ \hline

$\bullet$ Scalable Graph Processing Frameworks: A Taxonomy and Open Challenges (2018) \cite{2018SurveyScalable} & \makecell{TGC\\Distributed System} & \makecell{Partition\\Reorganization}\\ \hline

$\bullet$ A Survey of Field Programmable Gate Array (FPGA)-based Graph Convolutional Neural Network Accelerators: Challenges and Opportunities (2022) \cite{2022GCNFPGAsurvey} & \makecell{GNN\\FPGA} & \makecell{Partition\\Sampling\\Quantification} \\ \hline

$\bullet$ Computing Graph Neural Networks: A Survey from Algorithms to Accelerators (2021) \cite{2021GNNAlgToAccSurvey} & \makecell{GNN\\Algorithm \& Hardware} & \makecell{Many}\\ \hline

$\bullet$ Bottleneck Analysis of Dynamic Graph Neural Network Inference on CPU and GPU (2022) \cite{2022bottleneckDGNN} & \makecell{Dynamic GNN\\ CPU \& GPU} & \makecell{Partition\\Sampling}\\ \hline

$\bullet$ Scalable Graph Neural Network Training: The Case for Sampling (2021) \cite{2021GNNTrainingSurvey-full-mini} & \makecell{GNN\\Algorithm} & \makecell{Partition\\Sampling} \\ \hline

$\bullet$ Distributed Graph Neural Network Training: A Survey (2022) \cite{2022DistributedGNNSurvey} & \makecell{GNN \\ CPU \& GPU} & \makecell{Partition\\Sampling}\\ \hline

$\bullet$ The Evolution of Distributed Systems for Graph Neural Networks and their Origin in Graph Processing and Deep Learning: A Survey (2023) \cite{2023DistGNN-DNN-Survey} & \makecell{GNN\\Distributed System} & \makecell{Partition\\Sampling} \\\hline

$\bullet$ Survey on Graph Neural Network Acceleration: An Algorithmic Perspective (2022) \cite{2022surveyGNNAcc-liu} & \makecell{GNN \\ Algorithm} & \makecell{Many}\\ \hline

$\bullet$ A Survey on Graph Neural Network Acceleration: Algorithms, Systems, and Customized Hardware (2023) \cite{2023surveyGNN-Algo-System-hardware} &  \makecell{GNN\\ Algorithm \& Hardware} & \makecell{Many} \\ \hline

$\bullet$ Survey and Taxonomy of Lossless Graph Compression and Space-Efficient Graph Representations (2018) \cite{2018NNCompressionSurvey} & \makecell{Graph\\Algorithm} & \makecell{Quantification} \\ \hline
$\bullet$ Streaming Graph Partitioning: An Experimental Study (2018) \cite{2018partitionstream} & \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}GNN\\Algorithm\end{tabular}} & \multirow{3}{*}{Partition}\\
$\bullet$ A Survey of Current Challenges in Partitioning and Processing of Graph Structured Data in Parallel and Distributed Systems (2020) \cite{2020surveyPartition} &  &  \\ \hline

$\bullet$ Sampling Methods For Efficient Training of Graph Convolutional Networks: A Survey (2021) \cite{2021liu-sampling-survey} & \makecell{GNN \\ Algorithm} & \makecell{Sampling}\\ \hline
\end{tabular}
\vspace{-0.5cm}  %调整表格与下文距离
\end{table*}


\begin{table*}[h]
\vspace{-0.2cm}  %调整表格与上文距离
\caption{Works with GPP methods for Efficient Computing}
\vspace{-0.3cm}  %调整表格标题距离
\label{table:Efficient-computing}
%\renewcommand{\arraystretch}{1.2}%调行距
\setlength\tabcolsep{10pt}%调列距
\begin{tabular}{|c|c|c|p{7.8cm}|}
\hline
\textbf{Effect}  & \textbf{Method}   & \textbf{Alg.}     & \textbf{\makecell[c]{Works}}     \\
\hline
\multirow{2}{*}{\makecell{Load\\Balance}}        
& \multirow{2}{*}{Partition} & TGC & Pregel \cite{2010Pregel}, Giraph \cite{2011Giraph}, Mizan \cite{2013Mizan}, PowerGraph \cite{2012powergraph}, GraphLab \cite{2012graphlab}, PowerLyra \cite{2019powerlyra} \\ \cline{3-4}
&                            & GNN         & AliGraph \cite{2019Aligraph}, DistDGL\cite{2020DistDGL}, PaGraph\cite{2020PaGraph}, Dorylus \cite{2021Dorylus}, QGTC \cite{2022QGTC} \\
\hline
\multirow{4}{*}{\makecell{Reduce\\ Computation}}
& Sampling       & GNN & AliGraph \cite{2019Aligraph}, DistDGL \cite{2020DistDGL}, AGL \cite{2020AGL}, PaGraph \cite{2020PaGraph}, 2PGraph \cite{2021-2PGraph}, P3 \cite{2021P3}, DistDGLv2 \cite{2022DistDGLv2}, DGTP \cite{2022DGTP}, Pasca \cite{2022Pasca}, QGTC \cite{2022QGTC}, Sugar \cite{2023Sugar} \\
\cline{2-4}
& Sparsification & GNN & GLT\cite{2021GLT}, DyGNN \cite{2021DyGNN} \\
\cline{2-4}
& Reconstruction & GNN & GraphACT\cite{2020GraphACT}, GCNInfer\cite{2020GcnInference}, HAG\cite{2020Redundancy-free}, I-GCN\cite{2021I-gcn}, ReGNN\cite{2022ReGNN}  \\
\cline{2-4}
& Quantization   & GNN & FPGAN \cite{2020FPGAN}, Bi-GCN\cite{2021Bi-GCN}, QGTC \cite{2022QGTC}    \\
\hline
\end{tabular}
\vspace{-0.5cm}  %调整表格与下文距离
\end{table*}

==> old/taxonomy_old.tex <==
% methodology and taxonomy about 3 pages
%% 两种预优化策略：1. 改变图结构； 2. 改变数据结构
%% 6 种预处理方法：sampling，sparsification, partition, compression, reconstruction, reorder
%% 问题：partition似乎没有改变图的拓扑，只是进行了分割？？
%% 问题：reconstruction合并了重复使用的点和边，改变了图的拓扑结构，应该划分到 graph-structure里面
In this section,  we propose a taxonomy of existing preprocessing methods with double-decision by optimization targets and optimization strategies, as illustrated Figure \ref{fig:taxonomy}. Guided by the challenges encountered in graph processing acceleration, the optimization targets are classified into 4 categories: efficient computing, efficient data movement, efficient storage, and efficient communication (Figure \ref{fig:taxonomy}(b)). To achieve these targets, existing accelerating strategies are carried out through modifying graph structure and data structure, which contains 6 preprocessing methods: sampling, sparsification, partition, compression, reconstruction and reorder. Next, we elaborate on these preprocessing methods with examples in Section \ref{Graph Preprocessing Methods} and describe the optimization targets with details in next Section \ref{Optimization Targets of acceleration}.

%To achieve these targets, existing accelerating strategies are carried out through 6 graph preprocessing methods of sampling, sparsification, partiton, compression, reconstruction and reorder. Next, we elaborate on these preprocessing methods with examples in Section \ref{Graph Preprocessing Methods} and describe the optimization targets with details in next Section \ref{Optimization Targets of acceleration}.

\begin{figure}[ht]
    \centering
    \vspace{-0.2cm}  %调整图片与上文的垂直距离
    \setlength{\abovecaptionskip}{0.cm}     %调整图片标题与图距离
    \setlength{\belowcaptionskip}{-0.2cm}   %调整图片标题与下文距离
    \includegraphics[width=\textwidth]{fig/global-taxonomy.eps}
    \caption{Taxonomy of preprocessing methods for graph processing acceleration: (a) Graph Preprocessing Methods; (b) Optimization Targets.}
    \label{fig:taxonomy}
\end{figure}

%---------------------------------------------------------------------------------------------
%%%%% 预处理方法
%---------------------------------------------------------------------------------------------
\subsection{Graph Preprocessing Methods} \label{Graph Preprocessing Methods}

%% Graph-structure 主要改变图的拓扑结构或图的密度
%% Data-structure 主要改变数据结构或减小数据规模
As illustrated in Figure \ref{fig:taxonomy}(a), the six graph preprocessing methods are grouped into two categories according to the processing object. "Graph structure" denotes that the preprocessing methods mainly achieves acceleration by transforming the topology of graph or modifying the density of graph. "Data structure" denotes that preprocessing methods mainly achieves acceleration by converting the data structure or reducing data scale. The six methods elaborate respectively below core mechanisms and optimization effects.

%%%%%%-------- graph structure --------
%% 图片 Graph-structure：Sample, Sparsification, Partition, reconstruction
\begin{figure}[ht]
    \centering
    \vspace{-0.2cm}  %调整图片与上文的垂直距离
    \setlength{\abovecaptionskip}{0.cm}     %调整图片标题与图距离
    \setlength{\belowcaptionskip}{-0.2cm}   %调整图片标题与下文距离
    \includegraphics[width=\textwidth]{fig/graph-method.eps}
    \caption{Methods of modifying Graph-structure : (a) Sampling method; (b) Sparsification method; (c) Partition method; (d) Reconstruction method}
    \label{fig:graph-method}
\end{figure}

%-------- sampling ----------
\textcircled{a} \textbf{Sampling}
% 采样是一种通过选择节点创建子图的过程
% 采样是选择图中一层中的部分节点来获取子图用于后续训练，它来自于DNN的mini-batch
% 效果：efficient computation：采样增加随机性，提高收敛速度，进而提高计算效率
%       efficient data movement：mini-batch减少了每次计算的数据量，on-chip buffer 可以放下，减少了频繁的不规则的片外访存，xxxxxx。

Sampling is the process of creating subgraphs by selecting vertices. Similar to DNNs, GNNs training is usually executed with mini-batch manner especially GCNs. As illustrated in Figure \ref{fig:graph-method}(a), part of target vertex neighbors are selected to create subgraphs, which forms mini-batches for subsequent training. 

Sampling provides both \textbf{efficient computation} and \textbf{efficient data movement}. On the one hand, the randomness brought by sampling speeds up training convergence, which improves computing efficiency.  On the other hand, less data of mini-batch need to be cached in memory compared with full-batch, which reduces data movement between memory and storage. 

%-------- sparsification --------
\textcircled{b} \textbf{Sparsification}
% 稀疏化是一种去除冗余数据的过程，多用于动态图算法。（注意：稀疏化主要是针对输入图的稀疏化，这个应该不叫剪枝，剪枝会改变模型）
% eg: DyGNN，冗余消除，剪枝顶点和边。Drop edge等
%在计算过程中，一些顶点会提前收敛，多次迭代时造成冗余计算，在聚合时存在大量冗余边，如一个顶点和邻居特征十 分相似，那么这个邻居就不会有任何贡献，是冗余计算。

Sparsification is the process of removing redundant data, which is a classic method to accelerate dynamic graph algorithms. In the execution process, some vertices will converge ahead, causing redundant computing during multiple iterations. Some vertex features are similar to their neighbors, which takes no contribution when aggregating. These vertices and edges are the redundant data.  Figure \ref{fig:graph-method}(b) illustrated an edge-removing process,  task-irrelevant edges are removed with a specific metric. 

Sparsification method provides \textbf{efficient computation}, \textbf{efficient data movement} and \textbf{efficient storage}. Using sparse graphs reduces a lot of redundant computation and off-chip memory access, which not only saves communication bandwidth, but also reduces the storage usage.

%--------- partition --------
\textcircled{c} \textbf{Partition}
% 划分是将原始图分割为多个子图并在多个节点上进行计算的过程。
% 划分图，Foregraph，graphchi，graphicionado等利用interval and shard划分图
% 减少通信，提高局部性

Partition is the process of dividing the original graph into several subgraphs that are used for computing on one or multiple nodes. Figure \ref{fig:graph-method}(c) illustrates an example of graph partitioning with vertex-cut strategy in which the original graph is divided into three exclusive subgraphs using vertex replication.

Partition method provides \textbf{efficient computation}, \textbf{efficient data movement} and \textbf{efficient communication}. Some partition methods generate more localized subgraphs through clustering, reducing data movement between storages and improving load balancing. Some partition methods divide the original graph into independent subgraphs, decreasing the communication overhead in multi-node systems.

%---------- reconstruction ---------
\textcircled{d} \textbf{Reconstruction}
%%%% 定义：合并可以reuse的点和边，减少冗余计算，提高reuse效率
% Redundant-free：（在聚合时使用重构的新数据结构）输入图数据重构，合并点和边，redundant-free 找到可重复使用的可用中间结果，在 HAG 中为它们创建一个节点（合并）。
% I-GCN：先bfs聚簇，然后将可以reuse的点进行合并。提高局部性减少冗余计算
% 减少冗余提高计算效率，提高存储效率
%Some papers reconstruct the original graph data and propose their own data structures. 

Reconstruction is the process of merging vertex and edges as shown in Figure \ref{fig:graph-method}(d). The irregularity of graph data leads to amounts of redundant operation in accessing graph data. To solve this problem, a common method is to reconstruct the adjacency matrix, which efficiently improve data locality by merging similar vertex and edges.

Reconstruction method provides \textbf{efficient computation}, \textbf{efficient data movement}. Since reconstruction merges common neighbors, it reduces repetitive computing in aggregation. Meanwhile, merging improves the data locality, avoiding the data redundant movement caused by the poor reuse of on-chip data.


%%%%%%-------- data structure --------
%% 图片：Data-structure：Compresssion, Reorder
\begin{figure}[ht]
    \centering
    \vspace{-0.2cm}  %调整图片与上文的垂直距离
    \setlength{\abovecaptionskip}{0.cm}     %调整图片标题与图距离
    \setlength{\belowcaptionskip}{-0.2cm}   %调整图片标题与下文距离
    \includegraphics[width=\textwidth]{fig/data-method.eps}
    \caption{Methods of modifying data-structure : (a) Compression method; (b) Reorder method}
    \label{fig:data-method}
\end{figure}

%----------- compression ------------
\textcircled{e} \textbf{Compression}
% 对数据本身进行压缩，以更简洁的形式展示更多的信息
% 将复杂数据压缩为保留较少参数的轻量型数据的技术，
% 数据量化，sanger
Compression is the process of transformation of data to present it in a more compact form,in which quantization is one of the most classic technologies. As illustrated in Figure \ref{fig:data-method}(a), 32-bit float data is quantified to 2 bit unit data and the storage needed decreases 16 times. Though the data change, the loss of precision is usually acceptable due to the robust of graph model.

Data compression method provides \textbf{efficient computation}, \textbf{efficient data movement} and \textbf{efficient storage}. Quantization reduces the data amount and complexity, lowering the data movement cost and storage usage. More important, the complicated multiplication calculation can be transformed into simple shift operation when executing binarization quantified data, which effectively accelerates the computing efficiency.
%计算pattern 改变


\textcircled{f} \textbf{Reorder}
% reorder是一种通过对顶点重新排序进而优化数据布局的技术
% 局部性和index相关性更强，通过数据重排，在存储层面进行改变
% 通过顶点重排序进行的提前数据布局优化是一种广泛使用的技术，rabbit order，通过数据重排序提高数据局部性

Reorder is a method for optimizing data layout by modifying vertex arrangement. As illustrated in Figure \ref{fig:data-method}(b), the randomly ordered IDs in original graph are reordered into contiguous numbers in each community, and they make dense diagonal blocks (the shadowed squares in matrix). It's well perceived that the reordered matrix have dense diagonal blocks which means the improvement of data locality.

The reorder method provides \textbf{efficient computation} and \textbf{efficient data movement}. As mentioned above, the poor locality is a main obstacle to performance resulting from the unstructured topology of graph. Reordering vertex makes data cram tighter in memory without changing graph topology, which is a different way to improve locality compared to reconstruction method.

%---------------------------------------------------------------------------------------------
%%%% 优化目标
%---------------------------------------------------------------------------------------------
\subsection{Optimization Targets of acceleration} \label{Optimization Targets of acceleration}

% 如图5所示，加速主要从......四个方面进行优化。下面，将从硬件执行的角度，来介绍实际的硬件作用对象（对硬件执行的实际作用效果）。具体的paper与分析将在下一节进行详细的分类阐述。

As illustrated in Figure \ref{fig:taxonomy}(b), 

\blackcircled{a} efficient computing



\blackcircled{b} efficient data movement


\blackcircled{c} efficient storage


\blackcircled{d} efficient communication




% we classify the optimization factors and preprocessing methods via double-level taxonomy. The optimization factors are divided into 4 categories according to the hardware level, and are further subdivided into 13 sub-categories considering the specific effects. For preprocessing methods, existing methods are classified into six categories and group them into two based on core mechanism (Section \ref{taxonomy}). 



% 先概述(b)和(c)
% 按目前文献的工作，优化目标主要有4中，主要实现方法有6种。简单阐述6种方法是什么。

% 子章节：介绍(c)，详细的图+例子
% 子章节：介绍(b),图+内容


% 从优化目标(c)的角度来划分，然后引出(b)图的方法。




